Unsupervised Pathology Detection: A Deep Dive Into the State of the Art

Deep unsupervised approaches are gathering increased attention for applications such as pathology detection and segmentation in medical images since they promise to alleviate the need for large labeled datasets and are more generalizable than their supervised counterparts in detecting any kind of rare pathology. As the Unsupervised Anomaly Detection (UAD) literature continuously grows and new paradigms emerge, it is vital to continuously evaluate and benchmark new methods in a common framework, in order to reassess the state-of-the-art (SOTA) and identify promising research directions. To this end, we evaluate a diverse selection of cutting-edge UAD methods on multiple medical datasets, comparing them against the established SOTA in UAD for brain MRI. Our experiments demonstrate that newly developed feature-modeling methods from the industrial and medical literature achieve increased performance compared to previous work and set the new SOTA in a variety of modalities and datasets. Additionally, we show that such methods are capable of benefiting from recently developed self-supervised pre-training algorithms, further increasing their performance. Finally, we perform a series of experiments in order to gain further insights into some unique characteristics of selected models and datasets. Our code can be found under https://github.com/iolag/UPD_study/.

==> tables/cxr_ccd.tex <==
% Version 3
\begin{table}[t]
\centering
\caption{Image-level anomaly detection performance of the compared methods on CheXpert after self-supervised pre-training.
The small numbers show the change compared to the results without self-supervised pre-training and are color-coded (green and red) if the change is statistically significant with $p < 0.05$ using a two-sided Welch's t-test over multiple random seeds.
}
\label{tab:cxr_ccd}
\resizebox{\linewidth}{!}{
    \begin{tabular}{clcccccccc} 
    \toprule
    \multicolumn{2}{c}{} & \multicolumn{2}{c}{\textbf{Pleural Effusion}} &  & \multicolumn{2}{c}{\textbf{\textbf{Opacity}}} &  & \multicolumn{2}{c}{\textbf{Enlarged Card.}}  \\ 
    \cmidrule(r{4pt}){1-2}\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}
    & Method & \api  & AUROC &  & \api  & AUROC &  & \api  & AUROC \\ 
    % Image-reconstruction
    \cmidrule(r{4pt}){1-2}\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}
    \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{IS}}}}
    & VAE & 0.56 \tp{.01} & 0.58 \tp{.01} &  & 0.52 \tp{.01} & 0.54 \tu{} &  & 0.56 \tu{} & 0.57 \tp{.01} \\
    & r-VAE & 0.52 \tu{} & 0.57 \tu{} &  & 0.47 \tu{} & 0.49 \tn{.01} &  & 0.52 \tu{} & 0.56 \tu{} \\
    & f-AnoGAN & 0.60 \tp{.01} & 0.62 \tp{.01} &  & 0.50 \tp{.01} & 0.52 \tp{.01} &  & 0.58 \tp{.01} & 0.60 \tp{.01} \\
    & H-TAE-S & N/A & N/A &  & N/A & N/A &  & N/A & N/A \\
    % Feature-modeling
    \cmidrule(r{4pt}){1-2}\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}
    \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{FS}}}}
    & FAE & \textbf{0.74} \tp{.01} & \textbf{0.78} \tp{.01} &  & \textbf{0.55} \tn{.02} & \textbf{0.58} \tn{.03} &  & \textbf{0.65} \tp{.02} & \textbf{0.68} \tp{.02} \\
    & PaDiM & 0.59 \tn{.02} & 0.63 \tn{.03} &  & 0.48 \tn{.02} & 0.49 \tn{.03} &  & 0.58 \tn{.02} & 0.60 \tn{.03} \\
    & CFLOW-AD & 0.58 \tn{.09} & 0.62 \tn{.11} &  & 0.47 \tn{.05} & 0.48 \tn{.06} &  & 0.58 \tn{.04} & 0.60 \tn{.06} \\
    & RD & 0.66 \tp{.01} & 0.69 \tn{.02} &  & \textbf{0.55} \tp{.01} & \textbf{0.58} \tu{} &  & 0.61 \tu{} & 0.62 \tn{.01} \\
    % Attention-based
    \cmidrule(r{4pt}){1-2}\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}
    \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{AB}}}}
    & ExpVAE & 0.48 \tn{.03} & 0.47 \tn{.05} &  & 0.51 \tn{.01} & 0.49 \tn{.02} &  & 0.49 \tn{.03} & 0.48 \tn{.04} \\
    & AMCons & 0.43 \tp{.04} & 0.40 \tp{.09} &  & 0.50 \tp{.01} & 0.52 \tp{.04} &  & 0.45 \tp{.04} & 0.43 \tp{.06} \\
    % Self supervised
    \cmidrule(r{4pt}){1-2}\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}
    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{S-S}}}}
    & PII & 0.65 \tp{.01} & 0.66 \tp{.01} &  & 0.52 \tn{.01} & 0.53 \tn{.01} &  & 0.58 \tp{.02} & 0.59 \tp{.03} \\
    & DAE & 0.62 \tn{.01} & 0.64 \tn{.01} &  & 0.52 \tu{} & 0.54 \tn{.01} &  & 0.58 \tu{} & 0.60 \tu{} \\
    & CutPaste & 0.55 \tn{.03} & 0.58 \tn{.01} &  & 0.52 \tn{.01} & 0.54 \tu{} &  & 0.55 \tn{.02} & 0.56 \tn{.02} \\
    \cmidrule(r{4pt}){1-2}\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}
    & Random & 0.50 & 0.50 &  & 0.50 & 0.50 &  & 0.50 & 0.50 \\
    \bottomrule
    \end{tabular}}
\end{table}


% Version 2
% \begin{table}[t]
% \centering
% \caption{Image-level anomaly detection performance of the compared methods on CheXpert after self-supervised pre-training.}
% \label{tab:cxr_ccd}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{clcccccccc} 
% \toprule
% \multicolumn{2}{c}{} & \multicolumn{2}{c}{\textbf{Pleural Effusion}} &  & \multicolumn{2}{c}{\textbf{\textbf{Opacity}}} &  & \multicolumn{2}{c}{\textbf{Enlarged Card.}}  \\ 
% \cmidrule(r{4pt}){1-2}\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}
% & Method & \api  & AUROC &  & \api  & AUROC &  & \api  & AUROC \\ 
% % Image-reconstruction
% \cmidrule(r{4pt}){1-2}\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{IS}}}}
% & VAE & 0.56 & 0.58 &  & 0.52 & 0.54 &  & 0.56 & 0.57 \\
% & r-VAE & 0.52 & 0.57 &  & 0.47 & 0.49 &  & 0.52 & 0.56 \\
% & f-AnoGAN & 0.60 & 0.62 &  & 0.50 & 0.52 &  & 0.58 & 0.60 \\
% & H-TAE-S &N/A & N/A &  & N/A & N/A &  & N/A & N/A\\
% % Feature-modeling
% \cmidrule(r{4pt}){1-2}\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{FS}}}}
% & FAE & \textbf{0.74} & \textbf{0.78} &  & \textbf{0.55} & \textbf{0.58} &  & \textbf{0.65} & \textbf{0.68} \\
% & PaDiM & 0.59 & 0.63 &  & 0.48 & 0.49 &  & 0.58 & 0.60 \\
% & CFLOW-AD & 0.58 & 0.62 &  & 0.47 & 0.48 &  & 0.58 & 0.60 \\
% & RD & 0.66 & 0.69 &  & \textbf{0.55} & \textbf{0.58} &  & 0.61 & 0.62 \\
% % Attention-based
% \cmidrule(r{4pt}){1-2}\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}
% \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{AB}}}}
% & ExpVAE &0.48 & 0.47 &  & 0.51 & 0.49 &  & 0.49 & 0.48\\
% & AMCons & 0.43 & 0.40 &  & 0.50 & 0.52 &  & 0.45 & 0.43 \\
% % Self supervised
% \cmidrule(r{4pt}){1-2}\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}
% \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{S-S}}}}
% & PII & 0.65 & 0.66 &  & 0.52 & 0.53 &  & 0.58 & 0.59 \\
% & DAE & 0.62 & 0.64 &  & 0.52 & 0.54 &  & 0.58 & 0.60 \\
% & CutPaste & 0.55 & 0.58 &  & 0.52 & 0.54 &  & 0.55 & 0.56\\
% \cmidrule(r{4pt}){1-2}\cmidrule{3-4}\cmidrule{6-7}\cmidrule{9-10}
% & Random & 0.50 & 0.50 &  & 0.50 & 0.50 &  & 0.50 & 0.50 \\
% \bottomrule
% \end{tabular}}
% \end{table}


% \begin{table}[t]
% \centering
% \caption{Image-level Anomaly detection performance of the compared methods on CheXpert after self-supervised pre-training.}
% \label{tab:cxr_ccd}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lcccccccc} 
% \toprule
% \multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{Pleural Effusion}} &  & \multicolumn{2}{c}{\textbf{\textbf{Opacity}}} &  & \multicolumn{2}{c}{\textbf{Enlarged Card.}}  \\ 
% \cmidrule(r{4pt}){1-1}\cmidrule{2-3}\cmidrule{5-6}\cmidrule{8-9}
% Method & \api  & AUROC &  & \api  & AUROC &  & \api  & AUROC \\ 
% \cmidrule(r{4pt}){1-1}\cmidrule{2-3}\cmidrule{5-6}\cmidrule{8-9}
% VAE & 0.56 & 0.58 &  & 0.52 & 0.54 &  & 0.56 & 0.57 \\
% r-VAE & 0.52 & 0.57 &  & 0.47 & 0.49 &  & 0.52 & 0.56 \\
% f-AnoGAN & 0.60 & 0.62 &  & 0.50 & 0.52 &  & 0.58 & 0.60 \\
% AMCons & 0.43 & 0.40 &  & 0.50 & 0.52 &  & 0.45 & 0.43 \\
% FAE & \textbf{0.74} & \textbf{0.78} &  & \textbf{0.55} & \textbf{0.58} &  & \textbf{0.65} & \textbf{0.68} \\
% % DFR & 0.51 & 0.52 &  & 0.45 & 0.45 &  & 0.53 & 0.54 \\
% PaDiM & 0.59 & 0.63 &  & 0.48 & 0.49 &  & 0.58 & 0.60 \\
% CFLOW-AD & 0.58 & 0.62 &  & 0.47 & 0.48 &  & 0.58 & 0.60 \\
% RD & 0.66 & 0.69 &  & \textbf{0.55} & \textbf{0.58} &  & 0.61 & 0.62 \\
% PII & 0.65 & 0.66 &  & 0.52 & 0.53 &  & 0.58 & 0.59 \\
% DAE & 0.62 & 0.64 &  & 0.52 & 0.54 &  & 0.58 & 0.60 \\
% Random & 0.50 & 0.50 &  & 0.50 & 0.50 &  & 0.50 & 0.50 \\
% \bottomrule
% \end{tabular}}
% \end{table}

==> tables/cxr_ccd_std.tex <==
\begin{table*}[!t]
\centering
\caption{CXR results, with pre-training.}
\label{tab:cxr_ccd_std}
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{lcccccccc} 
\toprule
\multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{Pleural Effusion}} &  & \multicolumn{2}{c}{\textbf{\textbf{Opacity}}} &  & \multicolumn{2}{c}{\textbf{Enlarged Card.}}  \\ 
\cmidrule(r{4pt}){1-1}\cmidrule{2-3}\cmidrule{5-6}\cmidrule{8-9}
Method & AP\textsubscript{i}  & AUROC                                  &  & AP\textsubscript{i}  & AUROC                                  &  & AP\textsubscript{i}  & AUROC                                                          \\ 
\cmidrule(r{4pt}){1-1}\cmidrule{2-3}\cmidrule{5-6}\cmidrule{8-9}
VAE                  & 0.56 & 0.58                                   &  & 0.52 & 0.54                                   &  & 0.56 & 0.57                                                             \\
r-VAE                & 0.52 & 0.57                                   &  & 0.47 & 0.49                                   &  & 0.52 & 0.56                                                             \\
f-AnoGAN             & 0.61 & 0.63                                   &  & 0.50 & 0.52                                   &  & 0.59 & 0.60                                                             \\
PaDiM                & 0.59 & 0.63                                   &  & 0.48 & 0.49                                   &  & 0.58 & 0.60                                                             \\
FAE                  & 0.74 & 0.78                                   &  & 0.55 & 0.58                                   &  & 0.65 & 0.68                                                             \\
CFLOW-AD             & 0.58 & 0.62                                   &  & 0.47 & 0.48                                   &  & 0.58 & 0.60                                                             \\
RD                   & 0.66 & 0.69                                   &  & 0.55 & 0.58                                   &  & 0.61 & 0.62                                                             \\
% DFR                  & 0.52 & 0.54                                   &  & 0.45 & 0.46                                   &  & 0.53 & 0.55                                                             \\
PII                  & 0.66 & 0.68                                   &  & 0.55 & 0.56                                   &  & 0.58 & 0.59                                                             \\
DAE                  & 0.00 & 0.00                                   &  & 0.00 & 0.00                                   &  & 0.00 & 0.00                                                             \\
Random               & 0.50 & 0.50                                   &  & 0.50 & 0.50                                   &  & 0.50 & 0.50                                                             \\
\bottomrule
\end{tabular}}
\end{table*}

==> tables/cxr_std.tex <==
\begin{table*}[!t]
\centering
\caption{CXR results.}
\label{tab:cxr_std}
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{lcccccccc} 
\toprule
\multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{Pleural Effusion}} &  & \multicolumn{2}{c}{\textbf{\textbf{Opacity}}} &  & \multicolumn{2}{c}{\textbf{\textbf{\textbf{\textbf{Enlarged Card.}}}}}  \\ 
\cmidrule(r{4pt}){1-1}\cmidrule{2-3}\cmidrule{5-6}\cmidrule{8-9}
Method & AP\textsubscript{i}  & AUROC                                  &  & AP\textsubscript{i}  & AUROC                                  &  & AP\textsubscript{i}  & AUROC                                                          \\ 
\cmidrule(r{4pt}){1-1}\cmidrule{2-3}\cmidrule{5-6}\cmidrule{8-9}
VAE                  & 0.55 & 0.57                                   &  & 0.51 & 0.54                                   &  & 0.56 & 0.56                                                             \\
r-VAE                & 0.52 & 0.57                                   &  & 0.47 & 0.50                                   &  & 0.52 & 0.56                                                             \\
f-AnoGAN             & 0.59 & 0.61                                   &  & 0.49 & 0.51                                   &  & 0.57 & 0.59                                                             \\
PaDiM                & 0.61 & 0.66                                   &  & 0.50 & 0.52                                   &  & 0.60 & 0.63                                                             \\
FAE                  & 0.73 & 0.77                                   &  & 0.57 & 0.61                                   &  & 0.63 & 0.66                                                             \\
CFLOW-AD             & 0.67 & 0.73                                   &  & 0.52 & 0.54                                   &  & 0.62 & 0.66                                                             \\
RD                   & 0.65 & 0.71                                   &  & 0.54 & 0.58                                   &  & 0.61 & 0.63                                                             \\
% DFR                  & 0.56 & 0.60                                   &  & 0.47 & 0.49                                   &  & 0.57 & 0.60                                                             \\
PII                  & 0.69 & 0.70                                   &  & 0.56 & 0.57                                   &  & 0.58 & 0.59                                                             \\
DAE                  & 0.62 & 0.65                                   &  & 0.52 & 0.55                                   &  & 0.58 & 0.60                                                             \\
Random               & 0.50 & 0.50                                   &  & 0.50 & 0.50                                   &  & 0.50 & 0.50                                                             \\
\bottomrule
\end{tabular}}
\end{table*}

==> tables/main.tex <==

\begin{table*}
\centering
\caption{Detection and localization results of selected methods on the MRI and RF datasets.}
\label{tab:main}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccccccccccccc}
\toprule
 & \multicolumn{4}{c}{\textbf{ATLAS}} &  & \multicolumn{4}{c}{\textbf{BraTS-T1}} &  & \multicolumn{4}{c}{\textbf{BraTS-T2}} &  & \multicolumn{4}{c}{\textbf{DDR}}\\
\cmidrule(r{4pt}){1-1}\cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}\cmidrule{17-20}
Method & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize} & \begin{scriptsize}$\lceil$Dice$\rceil$ \end{scriptsize}&  & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize} & \begin{scriptsize}$\lceil$Dice$\rceil$ \end{scriptsize}&  & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize} & \begin{scriptsize}$\lceil$Dice$\rceil$ \end{scriptsize}&  & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize} & \begin{scriptsize}$\lceil$Dice$\rceil$ \end{scriptsize}\\
\cmidrule(r{4pt}){1-1}\cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}\cmidrule{17-20}
VAE      & 0.64 & 0.80  & 0.18 & 0.28                 &  & 0.64 & 0.70  & 0.13 & 0.19                 &  & 0.68 & 0.73  & 0.28 & 0.33                 &  & 0.48 & 0.48  & 0.02  & 0.05                  \\
r-VAE    & \textbf{0.68} & \textbf{0.83}  & 0.17 & 0.26                 &  & 0.70 & 0.76  & 0.13 & 0.19                 &  & 0.75 & 0.77  & 0.36 & 0.40                 &  & 0.52 & 0.50  & 0.03  & 0.09                  \\
f-AnoGAN & 0.21 & 0.39  & 0.02 & 0.05                 &  & 0.48 & 0.53  & 0.06 & 0.12                 &  & 0.56 & 0.61  & 0.15 & 0.21                 &  & 0.44 & 0.45  & 0.01  & 0.01                  \\
AMCons   & 0.33 & 0.65  & 0.01 & 0.02                 &  & 0.61 & 0.64  & 0.05 & 0.12                 &  & 0.78 & 0.78  & 0.35 & 0.40                 &  & 0.49 & 0.49  & 0.004 & 0.01                  \\
FAE      & 0.49 & 0.72  & 0.15 & 0.27                 &  & \textbf{0.86} & \textbf{0.85}  & \textbf{0.42} & \textbf{0.45}                 &  & \textbf{0.87} & \textbf{0.87}  & \textbf{0.51} & \textbf{0.52}                 &  & 0.64 & 0.63  & 0.07  & 0.15                  \\
DFR      & 0.34 & 0.59  & 0.07 & 0.15                 &  & 0.58 & 0.64  & 0.19 & 0.27                 &  & 0.67 & 0.69  & 0.34 & 0.37                 &  & 0.56 & 0.53  & 0.06  & 0.14                  \\
PaDiM    & 0.33 & 0.59  & 0.08 & 0.18                 &  & 0.60 & 0.65  & 0.21 & 0.28                 &  & 0.66 & 0.68  & 0.34 & 0.38                 &  & 0.55 & 0.55  & 0.02  & 0.07                  \\
CFLOW-AD & 0.34 & 0.59  & 0.05 & 0.11                 &  & 0.65 & 0.69  & 0.16 & 0.24                 &  & 0.71 & 0.72  & 0.31 & 0.35                 &  & 0.51 & 0.51  & 0.03  & 0.08                  \\
RD       & 0.60 & 0.78  & \textbf{0.25} & \textbf{0.36}                &  & 0.81 & 0.83  & 0.36 & 0.42                 &  & 0.85 & 0.85  & 0.47 & 0.50                 &  & \textbf{0.66} & \textbf{0.64}  & \textbf{0.10}  & \textbf{0.19}                  \\
PII      & 0.35 & 0.59  & 0.02 & 0.07                 &  & 0.54 & 0.64  & 0.13 & 0.22                 &  & 0.57 & 0.62  & 0.13 & 0.22                 &  & 0.62 & 0.63  & 0.01  & 0.01                  \\
DAE      & 0.37 & 0.63  & 0.07 & 0.14                 &  & 0.70 & 0.74  & 0.13 & 0.20                 &  & 0.81 & 0.80  & 0.47 & 0.49                 &  & 0.54 & 0.55  & 0.01  & 0.03                  \\
Random   & 0.26 & 0.50  & 0.01 & 0.02                 &  & 0.48 & 0.50  & 0.06 & 0.11                 &  & 0.48 & 0.50  & 0.06 & 0.11                 &  & 0.50 & 0.50  & 0.004 & 0.01                  \\
\bottomrule
\end{tabular}}
\end{table*}




==> tables/main_std.tex <==
% \begin{table*}[t]
% \centering
% \caption{Detection and localization results with standard deviation of selected methods on the MRI datasets.}
% \label{tab:main_std}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lcccccccccccccccccccc}
% \toprule
%  & \multicolumn{4}{c}{\textbf{BraTS-T2}} &  & \multicolumn{4}{c}{\textbf{BraTS-T1}} &  & \multicolumn{4}{c}{\textbf{ATLAS}} &  & \multicolumn{4}{c}{\textbf{DDR}} \\
% \cmidrule(r{4pt}){1-1}\cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}\cmidrule{17-20}
% Method & \api & AUROC & \app & \dice &  & \api & AUROC & \app & \dice &  & \api & AUROC & \app & \dice &  & \api & AUROC & \app & \dice & \\
% \cmidrule(r{4pt}){1-1}\cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}\cmidrule{17-20}
% VAE & 68$\pm$2 & 73$\pm$1 & 28$\pm$2 & 33$\pm$1 &  & 64$\pm$1 & 70$\pm$1 & 13$\pm$1 & 19$\pm$1 &  & 57$\pm$2 & 76$\pm$1 & 11$\pm$2 & 20$\pm$1 &  & 48$\pm$2 & 48$\pm$1 & 2$\pm$0 & 5$\pm$0 \\
% r-VAE & 75$\pm$0 & 77$\pm$0 & 36$\pm$1 & 40$\pm$1 &  & \\
% \bottomrule
% \end{tabular}}
% \end{table*}




\begin{table*}[t]
\centering
\caption{Detection and localization results with standard deviation of selected methods on the MRI datasets.}
\label{tab:main_std}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccccccccccccc}
\toprule
 & \multicolumn{4}{c}{\textbf{ATLAS}} &  & \multicolumn{4}{c}{\textbf{BraTS-T1}} &  & \multicolumn{4}{c}{\textbf{BraTS-T2}} \\
\cmidrule(r{4pt}){1-1}\cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}
Method & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize} & \begin{scriptsize}$\lceil$Dice$\rceil$ \end{scriptsize}&  & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize} & \begin{scriptsize}$\lceil$Dice$\rceil$ \end{scriptsize}&  & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize}& \begin{scriptsize}$\lceil$Dice$\rceil$ \end{scriptsize}\\
\cmidrule(r{4pt}){1-1}\cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}
VAE      & 0.57
  \begin{scriptsize}(0.02)\end{scriptsize}                    & 0.76 \begin{scriptsize}(0.01)\end{scriptsize}                    & 0.11 \begin{scriptsize}(0.01)\end{scriptsize}                  & 0.20 \begin{scriptsize}(0.02)\end{scriptsize}   & ~                     & 0.64
  \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.70
  \begin{scriptsize}(0.01)\end{scriptsize}                    & 0.13
  \begin{scriptsize}(0.01)\end{scriptsize}                 & 0.19
  \begin{scriptsize}(0.01)\end{scriptsize}                 & ~                     & 0.68
  \begin{scriptsize}(0.02)\end{scriptsize}                   & 0.73
  \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.28
  \begin{scriptsize}(0.02)\end{scriptsize}                 & 0.33
  \begin{scriptsize}(0.01)\end{scriptsize}                 \\
r-VAE    & 0.60
  \begin{scriptsize}(0.00)\end{scriptsize}                       & 0.78 \begin{scriptsize}(0.00)\end{scriptsize}                      & 0.09 \begin{scriptsize}(0.00)\end{scriptsize}                    & 0.17 \begin{scriptsize}(0.00)\end{scriptsize}   & ~                     & 0.70 \begin{scriptsize}(0.01)\end{scriptsize}                      & 0.76 \begin{scriptsize}(0.00)\end{scriptsize}                       & 0.13 \begin{scriptsize}(0.00)\end{scriptsize}                     & 0.19 \begin{scriptsize}(0.00)\end{scriptsize}                     & ~                     & 0.75 \begin{scriptsize}(0.00)\end{scriptsize}                       & 0.77 \begin{scriptsize}(0.00)\end{scriptsize}                       & 0.36 \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.40 \begin{scriptsize}(0.01)\end{scriptsize}                    \\
f-AnoGAN & 0.26
  \begin{scriptsize}(0.01)\end{scriptsize}                    & 0.46 \begin{scriptsize}(0.04)\end{scriptsize}                    & 0.02 \begin{scriptsize}(0.01)\end{scriptsize}                  & 0.06 \begin{scriptsize}(0.03)\end{scriptsize}  & ~                     & 0.48 \begin{scriptsize}(0.02)\end{scriptsize}                     & 0.53 \begin{scriptsize}(0.02)\end{scriptsize}                     & 0.06 \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.12 \begin{scriptsize}(0.01)\end{scriptsize}                   & ~                     & 0.56 \begin{scriptsize}(0.07)\end{scriptsize}                     & 0.61 \begin{scriptsize}(0.06)\end{scriptsize}                     & 0.15 \begin{scriptsize}(0.04)\end{scriptsize}                   & 0.21 \begin{scriptsize}(0.04)\end{scriptsize}                   \\
AMCons   & 0.32
  \begin{scriptsize}(0.02)\end{scriptsize} & \multicolumn{1}{l}{0.53 \begin{scriptsize}(0.02)\end{scriptsize}} & \multicolumn{1}{l}{0.01 \begin{scriptsize}(0.00)\end{scriptsize}} & 0.03 \begin{scriptsize}(0.00)\end{scriptsize}   & \multicolumn{1}{l}{~} & \multicolumn{1}{l}{0.61 \begin{scriptsize}(0.02)\end{scriptsize}} & \multicolumn{1}{l}{0.64 \begin{scriptsize}(0.02)\end{scriptsize}} & \multicolumn{1}{l}{0.05 \begin{scriptsize}(0.00)\end{scriptsize}} & \multicolumn{1}{l}{0.12 \begin{scriptsize}(0.00)\end{scriptsize}} & \multicolumn{1}{l}{~} & \multicolumn{1}{l}{0.78 \begin{scriptsize}(0.01)\end{scriptsize}} & \multicolumn{1}{l}{0.78 \begin{scriptsize}(0.01)\end{scriptsize}} & \multicolumn{1}{l}{0.35 \begin{scriptsize}(0.00)\end{scriptsize}} & \multicolumn{1}{l}{0.40 \begin{scriptsize}(0.00)\end{scriptsize}}  \\
FAE      & 0.50
  \begin{scriptsize}(0.00)\end{scriptsize}    & 0.73 \begin{scriptsize}(0.00)\end{scriptsize}                       & 0.08 \begin{scriptsize}(0.00)\end{scriptsize}                     & 0.18 \begin{scriptsize}(0.00)\end{scriptsize}   & ~                     & 0.86 \begin{scriptsize}(0.00)\end{scriptsize}                       & 0.85 \begin{scriptsize}(0.00)\end{scriptsize}                       & 0.42 \begin{scriptsize}(0.00)\end{scriptsize}                     & 0.45 \begin{scriptsize}(0.00)\end{scriptsize}                     & ~                     & 0.87 \begin{scriptsize}(0.00)\end{scriptsize}                       & 0.87 \begin{scriptsize}(0.00)\end{scriptsize}                       & 0.51 \begin{scriptsize}(0.00)\end{scriptsize}                     & 0.52 \begin{scriptsize}(0.00)\end{scriptsize}                     \\
% DFR      & 0.37
%   \begin{scriptsize}(0.01)\end{scriptsize} & 0.58 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.05 \begin{scriptsize}(0.00)\end{scriptsize}                     & 0.12 \begin{scriptsize}(0.00)\end{scriptsize}   & ~                     & 0.58 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.64 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.19 \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.27 \begin{scriptsize}(0.01)\end{scriptsize}                   & ~                     & 0.67 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.69 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.34 \begin{scriptsize}(0.00)\end{scriptsize}                     & 0.37 \begin{scriptsize}(0.00)\end{scriptsize}                     \\
PaDiM    & 0.34
  \begin{scriptsize}(0.04)\end{scriptsize} & 0.56 \begin{scriptsize}(0.04)\end{scriptsize}                     & 0.05 \begin{scriptsize}(0.00)\end{scriptsize}                     & 0.13 \begin{scriptsize}(0.01)\end{scriptsize} & ~                     & 0.60 \begin{scriptsize}(0.02)\end{scriptsize}                      & 0.65 \begin{scriptsize}(0.02)\end{scriptsize}                     & 0.21 \begin{scriptsize}(0.02)\end{scriptsize}                   & 0.28 \begin{scriptsize}(0.02)\end{scriptsize}                   & ~                     & 0.66 \begin{scriptsize}(0.02)\end{scriptsize}                     & 0.68 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.34 \begin{scriptsize}(0.02)\end{scriptsize}                   & 0.38 \begin{scriptsize}(0.01)\end{scriptsize}                   \\
CFLOW-AD & 0.40
  \begin{scriptsize}(0.02)\end{scriptsize}  & 0.62 \begin{scriptsize}(0.02)\end{scriptsize}                     & 0.04 \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.10 \begin{scriptsize}(0.02)\end{scriptsize}  & ~                     & 0.65 \begin{scriptsize}(0.06)\end{scriptsize}                     & 0.69 \begin{scriptsize}(0.06)\end{scriptsize}                     & 0.16 \begin{scriptsize}(0.03)\end{scriptsize}                   & 0.24 \begin{scriptsize}(0.04)\end{scriptsize}                   & ~                     & 0.71 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.72 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.31 \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.35 \begin{scriptsize}(0.00)\end{scriptsize}                     \\
RD        & 0.55
  \begin{scriptsize}(0.00)\end{scriptsize}   & 0.77 \begin{scriptsize}(0.00)\end{scriptsize}                       & 0.11 \begin{scriptsize}(0.00)\end{scriptsize}                     & 0.22 \begin{scriptsize}(0.00)\end{scriptsize}   & ~                     & 0.81 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.83 \begin{scriptsize}(0.00)\end{scriptsize}                       & 0.36 \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.42 \begin{scriptsize}(0.01)\end{scriptsize}                   & ~                     & 0.85 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.85 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.47 \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.50 \begin{scriptsize}(0.01)\end{scriptsize}                    \\
PII      & 0.37
  \begin{scriptsize}(0.04)\end{scriptsize} & 0.60 \begin{scriptsize}(0.03)\end{scriptsize}                      & 0.03 \begin{scriptsize}(0.00)\end{scriptsize}                     & 0.07 \begin{scriptsize}(0.01)\end{scriptsize} &  ~                     & 0.54 \begin{scriptsize}(0.03)\end{scriptsize}                     & 0.64 \begin{scriptsize}(0.03)\end{scriptsize}                     & 0.13 \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.22 \begin{scriptsize}(0.02)\end{scriptsize}                   & ~                     & 0.57 \begin{scriptsize}(0.07)\end{scriptsize}                     & 0.62 \begin{scriptsize}(0.09)\end{scriptsize}                     & 0.13 \begin{scriptsize}(0.04)\end{scriptsize}                   & 0.22 \begin{scriptsize}(0.05)\end{scriptsize}                   \\
DAE      & 0.44
  \begin{scriptsize}(0.02)\end{scriptsize} & 0.65 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.05 \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.13 \begin{scriptsize}(0.01)\end{scriptsize} & ~                     & 0.70 \begin{scriptsize}(0.01)\end{scriptsize}                      & 0.74 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.13 \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.20 \begin{scriptsize}(0.01)\end{scriptsize}                    & ~                     & 0.81 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.80 \begin{scriptsize}(0.01)\end{scriptsize}                      & 0.47 \begin{scriptsize}(0.02)\end{scriptsize}                   & 0.49 \begin{scriptsize}(0.01)\end{scriptsize}                   \\
Random   & 0.26                                                                                                  & 0.50                                                                                                & 0.01                                                                                              & 0.02                                                                                              &                       & 0.48                                                                                                & 0.50                                                                                                & 0.06                                                                                              & 0.11                                                                                              &                       & 0.48                                                                                                & 0.50                                                                                                & 0.06                                                                                              & 0.11                                                                                              \\
\bottomrule
\end{tabular}}
\end{table*}




==> tables/main_std_2.tex <==
% \usepackage{caption}
% \usepackage{booktabs}



\begin{table*}[t]
\centering
\caption{Detection and localization results with standard deviation of selected methods on the RF and CXR datasets.}
\label{tab:main_std_2}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccccccc} 
\toprule
 & \multicolumn{4}{c}{\textbf{DDR}}& \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{CheXpert - Pleural Effusion}}& & \multicolumn{2}{c}{\textbf{\textbf{CheXpert - Opacity}}}& \multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{CheXpert - Enlarged Card.}} \\ 
\cmidrule(r{4pt}){1-1}\cmidrule{2-5}\cmidrule{7-8}\cmidrule{10-11}\cmidrule{13-14}
Method & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize} & \begin{scriptsize}$\lceil$Dice$\rceil$\end{scriptsize}&& \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} && \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} \\ 
\cmidrule(lr){1-1}\cmidrule{2-5}\cmidrule{7-8}\cmidrule{10-11}\cmidrule{13-14}
VAE& 0.48
\begin{scriptsize}(0.02)\end{scriptsize} & 0.48
\begin{scriptsize}(0.01)\end{scriptsize} & 0.02
\begin{scriptsize}(0.00)\end{scriptsize} & 0.05
\begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.55
\begin{scriptsize}(0.00)\end{scriptsize} & 0.57
\begin{scriptsize}(0.01)\end{scriptsize} & ~ & 0.51
\begin{scriptsize}(0.00)\end{scriptsize} & 0.54
\begin{scriptsize}(0.01)\end{scriptsize} & ~& 0.56
\begin{scriptsize}(0.00)\end{scriptsize} & 0.56
\begin{scriptsize}(0.01)\end{scriptsize}\\
r-VAE& 0.51
\begin{scriptsize}(0.01)\end{scriptsize} & 0.50 \begin{scriptsize}(0.01)\end{scriptsize}& 0.03 \begin{scriptsize}(0.01)\end{scriptsize} & 0.08 \begin{scriptsize}(0.02)\end{scriptsize} & ~& 0.52
\begin{scriptsize}(0.00)\end{scriptsize} & 0.57 \begin{scriptsize}(0.00)\end{scriptsize} & ~ & 0.47 \begin{scriptsize}(0.00)\end{scriptsize} & 0.5 \begin{scriptsize}(0.01)\end{scriptsize}& ~& 0.52 \begin{scriptsize}(0.02)\end{scriptsize} & 0.56 \begin{scriptsize}(0.02)\end{scriptsize}\\
f-AnoGAN & 0.44
\begin{scriptsize}(0.02)\end{scriptsize} & 0.45 \begin{scriptsize}(0.01)\end{scriptsize} & 0.01 \begin{scriptsize}(0.00)\end{scriptsize} & 0.01 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.59
\begin{scriptsize}(0.00)\end{scriptsize} & 0.61 \begin{scriptsize}(0.00)\end{scriptsize} & ~ & 0.49 \begin{scriptsize}(0.01)\end{scriptsize} & 0.51 \begin{scriptsize}(0.02)\end{scriptsize} & ~& 0.57 \begin{scriptsize}(0.00)\end{scriptsize} & 0.59 \begin{scriptsize}(0.00)\end{scriptsize}\\
AMCons & 0.49
\begin{scriptsize}(0.00)\end{scriptsize} & 0.49 \begin{scriptsize}(0.00)\end{scriptsize} & 0.004 \begin{scriptsize}(0.00)\end{scriptsize} & 0.01 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.39
\begin{scriptsize}(0.01)\end{scriptsize} & 0.31 \begin{scriptsize}(0.03)\end{scriptsize} & ~ & 0.49 \begin{scriptsize}(0.02)\end{scriptsize} & 0.48 \begin{scriptsize}(0.03)\end{scriptsize} & ~& 0.41 \begin{scriptsize}(0.01)\end{scriptsize} & 0.37 \begin{scriptsize}(0.02)\end{scriptsize}\\
FAE& 0.64
\begin{scriptsize}(0.00)\end{scriptsize} & 0.63 \begin{scriptsize}(0.01)\end{scriptsize} & 0.07 \begin{scriptsize}(0.00)\end{scriptsize} & 0.15 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.73
\begin{scriptsize}(0.00)\end{scriptsize} & 0.77 \begin{scriptsize}(0.00)\end{scriptsize} & ~ & 0.57 \begin{scriptsize}(0.00)\end{scriptsize} & 0.61 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.63 \begin{scriptsize}(0.00)\end{scriptsize} & 0.66 \begin{scriptsize}(0.00)\end{scriptsize}\\
% DFR& 0.56
% \begin{scriptsize}(0.00)\end{scriptsize} & 0.53 \begin{scriptsize}(0.01)\end{scriptsize} & 0.06 \begin{scriptsize}(0.00)\end{scriptsize} & 0.14 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.56
% \begin{scriptsize}(0.00)\end{scriptsize} & 0.60 \begin{scriptsize}(0.00)\end{scriptsize}& ~ & 0.47 \begin{scriptsize}(0.00)\end{scriptsize} & 0.49 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.57 \begin{scriptsize}(0.00)\end{scriptsize} & 0.60 \begin{scriptsize}(0.00)\end{scriptsize} \\
PaDiM& 0.55
\begin{scriptsize}(0.02)\end{scriptsize} & 0.55 \begin{scriptsize}(0.02)\end{scriptsize} & 0.02 \begin{scriptsize}(0.00)\end{scriptsize} & 0.07 \begin{scriptsize}(0.01)\end{scriptsize} & ~& 0.61
\begin{scriptsize}(0.00)\end{scriptsize} & 0.66 \begin{scriptsize}(0.00)\end{scriptsize} & ~ & 0.50 \begin{scriptsize}(0.00)\end{scriptsize}& 0.52 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.60 \begin{scriptsize}(0.00)\end{scriptsize}& 0.63 \begin{scriptsize}(0.00)\end{scriptsize}\\
CFLOW-AD & 0.51
\begin{scriptsize}(0.01)\end{scriptsize} & 0.51 \begin{scriptsize}(0.02)\end{scriptsize} & 0.03 \begin{scriptsize}(0.00)\end{scriptsize} & 0.08 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.67
\begin{scriptsize}(0.00)\end{scriptsize} & 0.73 \begin{scriptsize}(0.00)\end{scriptsize} & ~ & 0.52 \begin{scriptsize}(0.00)\end{scriptsize} & 0.54 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.62 \begin{scriptsize}(0.00)\end{scriptsize} & 0.66 \begin{scriptsize}(0.00)\end{scriptsize}\\
RD & 0.66
\begin{scriptsize}(0.00)\end{scriptsize} & 0.64 \begin{scriptsize}(0.00)\end{scriptsize} & 0.10 \begin{scriptsize}(0.00)\end{scriptsize}& 0.19 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.65
\begin{scriptsize}(0.00)\end{scriptsize} & 0.71 \begin{scriptsize}(0.00)\end{scriptsize} & ~ & 0.54 \begin{scriptsize}(0.00)\end{scriptsize} & 0.58 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.61 \begin{scriptsize}(0.00)\end{scriptsize} & 0.63 \begin{scriptsize}(0.00)\end{scriptsize}\\
PII& 0.62
\begin{scriptsize}(0.03)\end{scriptsize} & 0.63 \begin{scriptsize}(0.02)\end{scriptsize} & 0.01 \begin{scriptsize}(0.00)\end{scriptsize} & 0.01 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.64
\begin{scriptsize}(0.05)\end{scriptsize} & 0.65 \begin{scriptsize}(0.04)\end{scriptsize} & ~ & 0.53 \begin{scriptsize}(0.03)\end{scriptsize} & 0.54 \begin{scriptsize}(0.04)\end{scriptsize} & ~& 0.56 \begin{scriptsize}(0.03)\end{scriptsize} & 0.56 \begin{scriptsize}(0.04)\end{scriptsize}\\
DAE& 0.54
\begin{scriptsize}(0.07)\end{scriptsize} & 0.55 \begin{scriptsize}(0.09)\end{scriptsize} & 0.01 \begin{scriptsize}(0.00)\end{scriptsize} & 0.03 \begin{scriptsize}(0.01)\end{scriptsize} & ~& 0.63
\begin{scriptsize}(0.00)\end{scriptsize} & 0.65 \begin{scriptsize}(0.00)\end{scriptsize} & ~ & 0.52 \begin{scriptsize}(0.01)\end{scriptsize} & 0.55 \begin{scriptsize}(0.01)\end{scriptsize} & ~& 0.58 \begin{scriptsize}(0.01)\end{scriptsize} & 0.60 \begin{scriptsize}(0.01)\end{scriptsize} \\
Random & 0.26& 0.50& 0.004 & 0.01&& 0.50& 0.50& & 0.50& 0.50&& 0.50& 0.50 \\
\bottomrule
\end{tabular}}
\end{table*}

==> tables/pretrain.tex <==


\begin{table*}
\centering
\caption{Detection and localization results of selected methods on the MRI and RF datasets after self-supervised pre-training.}
\label{tab:pretrain}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccccccccccccc}
\toprule
 & \multicolumn{4}{c}{\textbf{ATLAS}} &  & \multicolumn{4}{c}{\textbf{BraTS-T1}} &  & \multicolumn{4}{c}{\textbf{BraTS-T2}} &  & \multicolumn{4}{c}{\textbf{DDR}}\\
\cmidrule(r{4pt}){1-1}\cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}\cmidrule{17-20}
Method & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize} & \begin{scriptsize}$\lceil$Dice$\rceil$ \end{scriptsize}&  & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize} & \begin{scriptsize}$\lceil$Dice$\rceil$ \end{scriptsize}&  & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize} & \begin{scriptsize}$\lceil$Dice$\rceil$ \end{scriptsize}&  & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize} & \begin{scriptsize}$\lceil$Dice$\rceil$ \end{scriptsize}\\
\cmidrule(r{4pt}){1-1}\cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}\cmidrule{17-20}
VAE      & 0.64 & 0.80  & 0.18 & 0.28                 &  & 0.64 & 0.70  & 0.13 & 0.19                 &  & 0.68 & 0.73  & 0.27 & 0.33                 &  & 0.48 & 0.48  & 0.02  & 0.05                  \\
r-VAE    & \textbf{0.68} & \textbf{0.83}  & 0.17 & 0.26                 &  & 0.70 & 0.76  & 0.13 & 0.19                 &  & 0.75 & 0.77  & 0.36 & 0.40                 &  & 0.49 & 0.48  & 0.02  & 0.09                  \\
f-AnoGAN & 0.21 & 0.40  & 0.01 & 0.04                 &  & 0.48 & 0.53  & 0.06 & 0.11                 &  & 0.63 & 0.70  & 0.15 & 0.21                 &  & 0.41 & 0.42  & 0.01  & 0.01                  \\
AMCons   & 0.33 & 0.65  & 0.01 & 0.02                 &  & 0.61 & 0.64  & 0.06 & 0.12                 &  & 0.73 & 0.74  & 0.27 & 0.34                 &  & 0.49 & 0.50  & 0.004  & 0.01                  \\
FAE      & 0.52 & 0.74  & \textbf{0.19} & \textbf{0.31}                 &  & \textbf{0.85} & \textbf{0.85}  & \textbf{0.43} & \textbf{0.46}                 &  & \textbf{0.89} & \textbf{0.88}  &\textbf{0.55} & \textbf{0.55}                 &  & 0.55 & 0.57  & 0.03  & 0.08                  \\
% DFR      & 0.46 & 0.72  & 0.11 & 0.21                 &  & 0.73 & 0.77  & 0.32 & 0.37                 &  & 0.76 & 0.78  & 0.46 & 0.47                 &  & 0.53 & 0.50  & 0.03  & 0.08                  \\
PaDiM    & 0.44 & 0.71  & 0.09 & 0.17                 &  & 0.74 & 0.78  & 0.26 & 0.32                 &  & 0.81 & 0.81  & 0.47 & 0.48                 &  & 0.54 & 0.54  & 0.02  & 0.05                  \\
CFLOW-AD & 0.41 & 0.65  & 0.07 & 0.14                 &  & 0.76 & 0.78  & 0.24 & 0.30                 &  & 0.79 & 0.80  & 0.31 & 0.38                 &  & 0.53 & 0.54  & 0.02  & 0.07                  \\
RD       & 0.56 & 0.76  & 0.13 & 0.22                 &  & 0.74 & 0.78  & 0.28 & 0.35                 &  & 0.84 & 0.85  & 0.39 & 0.44                 &  & 0.53 & 0.54  & \textbf{0.04}  & 0.09                  \\
PII      & 0.27 & 0.49  & 0.01 & 0.03                 &  & 0.46 & 0.50  & 0.07 & 0.14                 &  & 0.60 & 0.66  & 0.11 & 0.19                 &  & \textbf{0.60} & \textbf{0.60}  & 0.01  & 0.04                  \\
DAE      & 0.42 & 0.66  & 0.10 & 0.17                 &  & 0.71 & 0.75  & 0.14 & 0.20                 &  & 0.81 & 0.81  & 0.48 & 0.50                 &  & 0.59 & \textbf{0.60}  & 0.01  & 0.03                  \\
Random   & 0.26 & 0.50  & 0.01 & 0.02                 &  & 0.48 & 0.50  & 0.06 & 0.11                 &  & 0.48 & 0.50  & 0.06 & 0.11                 &  & 0.50 & 0.50  & 0.004 & 0.01                  \\
\bottomrule
\end{tabular}}
\end{table*}





==> tables/pretrain_new.tex <==

% Version 3
\renewcommand{\row}[5]{#1 & #4 && #3 && #2 && #5}
\begin{table*}
\centering
\caption{Detection and localization results of the image-reconstruction (\textbf{IR}), feature-modeling (\textbf{FM}), attention-based (\textbf{AB}), and self-supervised anomaly detection (\textbf{S-S}) methods on the brain-MRI and RF datasets after self-supervised pre-training. The small numbers show the change compared to the results without self-supervised pre-training.}
\label{tab:pretrain}
\resizebox{\linewidth}{!}{
    \begin{tabular}{clccccccccccccccccccc}
        \toprule
        % Datasets
        & \row{}{\multicolumn{4}{c}{\textbf{ATLAS}}}{\multicolumn{4}{c}{\textbf{BraTS-T1}}}{\multicolumn{4}{c}{\textbf{BraTS-T2}}}{ \multicolumn{4}{c}{\textbf{DDR}}}\\
        \cmidrule(r{4pt}){1-2}\cmidrule{3-6}\cmidrule{8-11}\cmidrule{13-16}\cmidrule{18-21}
        % Metrics
        & & \multicolumn{2}{c}{image-level} & \multicolumn{2}{c}{pixel-level} && \multicolumn{2}{c}{image-level} & \multicolumn{2}{c}{pixel-level} && \multicolumn{2}{c}{image-level} & \multicolumn{2}{c}{pixel-level} && \multicolumn{2}{c}{image-level} & \multicolumn{2}{c}{pixel-level} \\[1mm]
        & Method & \api & AUROC & \app & \dice && \api & AUROC & \app & \dice && \api & AUROC & \app & \dice && \api & AUROC & \app & \dice \\
        \cmidrule(r{4pt}){1-2}\cmidrule{3-6}\cmidrule{8-11}\cmidrule{13-16}\cmidrule{18-21}
        % Image space methods
        \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{IR}}}}
        & \row{VAE}{0.57 \tu{} & 0.76 \tu{} & \textbf{0.11} \tu{} & 0.20 \tu{}}{0.64 \tu{} & 0.70 \tu{} & 0.13 \tu{} & 0.19 \tu{}}{0.68 \tu{} & 0.73 \tu{} & 0.27 \tn{.01} & 0.33 \tu{}}{0.48 \tu{} & 0.48 \tu{} & 0.02 \tu{} & 0.05 \tu{}} \\
        & \row{r-VAE}{\textbf{0.61} \tp{.01} & \textbf{0.79} \tp{.01} & 0.09 \tu{} & 0.17 \tu{}}{0.70 \tu{} & 0.76 \tu{} & 0.13 \tu{} & 0.19 \tu{}}{0.75 \tu{} & 0.77 \tu{} & 0.36 \tu{} & 0.40 \tu{}}{0.49 \tn{.03} & 0.48 \tn{.02} & 0.02 \tn{.01} & 0.09 \tu{}} \\
        & \row{f-AnoGAN}{0.28 \tp{.02} & 0.50 \tp{.04} & 0.02 \tu{} & 0.04 \tn{.02}}{0.48 \tu{} & 0.53 \tu{} & 0.06 \tu{} & 0.11 \tn{.01}}{0.63 \tp{.07} & 0.70  \tp{.09} & 0.15 \tu{} & 0.21 \tu{}}{0.41 \tn{.03} & 0.42 \tn{.03} & 0.01 \tu{} & 0.01 \tu{}} \\
        & \row{H-TAE-S}{N/A & N/A & N/A & N/A}{N/A & N/A & N/A & N/A}{N/A & N/A & N/A & N/A}{N/A & N/A & N/A & N/A} \\
        \cmidrule(r{4pt}){1-2}\cmidrule{3-6}\cmidrule{8-11}\cmidrule{13-16}\cmidrule{18-21}
        % Feature space methods
        \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{FM}}}}
        & \row{FAE}{0.53 \tp{.03} & 0.75 \tp{.02} & 0.10 \tp{.02} & \textbf{0.21} \tp{.03}}{\textbf{0.85} \tn{.01} & \textbf{0.85} \tu{} & \textbf{0.43} \tp{.01} & \textbf{0.46} \tp{.01}}{\textbf{0.89} \tp{.02} & \textbf{0.88} \tp{.01} &\textbf{0.55} \tp{.04} & \textbf{0.55} \tp{.03}}{0.55 \tn{.09} & 0.57 \tn{.06} & 0.03 \tn{.04} & 0.08 \tn{.07}} \\
        & \row{PaDiM}{0.41 \tp{.07} & 0.65 \tp{.09} & 0.07 \tp{.02} & 0.16 \tp{.03}}{0.74 \tp{.14} & 0.78 \tp{.13} & 0.26 \tp{.05} & 0.32 \tp{.04}}{0.81 \tp{.15} & 0.81 \tp{.13} & 0.47 \tp{.14} & 0.48 \tp{.10}}{0.54 \tn{.01} & 0.54 \tn{.01} & 0.02 \tu{} & 0.05 \tn{.02}} \\
        & \row{CFLOW-AD}{0.45 \tp{.05} & 0.68 \tp{.06} & 0.06 \tp{.02} & 0.14 \tp{.04}}{0.76 \tp{.11} & 0.78 \tp{.09} & 0.24 \tp{.08} & 0.30 \tp{.06}}{0.79 \tp{.08} & 0.80 \tp{.08} & 0.31 \tu{} & 0.38 \tp{.03}}{0.53 \tp{.02} & 0.54 \tp{.03} & 0.02 \tn{.01} & 0.07 \tn{.01}} \\
        & \row{RD}{0.42 \tn{.13} & 0.64 \tn{.13} & 0.05 \tn{.06} & 0.09 \tn{.13}}{0.74 \tn{.07} & 0.78 \tn{.05} & 0.28 \tn{.08} & 0.35 \tn{.07}}{0.84 \tn{.01} & 0.85 \tu{} & 0.39 \tn{.08} & 0.44 \tn{.06}}{0.53 \tn{.13} & 0.54 \tn{.10} & \textbf{0.04} \tn{.06} & 0.09 \tn{.10}} \\
        \cmidrule(r{4pt}){1-2}\cmidrule{3-6}\cmidrule{8-11}\cmidrule{13-16}\cmidrule{18-21}
        % Attention-based methods
        \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{AB}}}}
        & \row{ExpVAE} {0.40 \tp{.03} & 0.62 \tp{.05} & 0.01 \tu{} & 0.03 \tu{}}{0.58 \tp{.02} & 0.61 \tp{.05} & 0.05 \tn{.02} & 0.12 \tn{.01}}{0.66 \tp{.03} & 0.68 \tp{.02} & 0.15 \tp{.03} & 0.22 \tp{.04}}{0.52 \tn{.01} & 0.53 \tn{.01} & 0.004 \tu{} & 0.01 \tu{}}  \\
        & \row{AMCons}{0.31 \tn{.01} & 0.52 \tn{.01} & 0.01 \tu{} & 0.03 \tu{}}{0.61 \tu{} & 0.64 \tu{} & 0.06 \tp{.01} & 0.12 \tu{}}{0.73 \tn{.05} & 0.74 \tn{.04} & 0.27 \tn{.08} & 0.34 \tn{.06}}{0.49 \tu{} & 0.50 \tp{.01} & 0.004 \tu{} & 0.01 \tu{}} \\
        \cmidrule(r{4pt}){1-2}\cmidrule{3-6}\cmidrule{8-11}\cmidrule{13-16}\cmidrule{18-21}
        % Self-supervised methods
        \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{S-S}}}}
        & \row{PII}{0.32 \tn{.05} & 0.52 \tn{.08} & 0.02 \tn{.01} & 0.05 \tn{.02}}{0.46 \tn{.08} & 0.50 \tn{.14} & 0.07 \tn{.06} & 0.14 \tn{.08}}{0.60 \tp{.03} & 0.66 \tp{.04} & 0.11 \tn{.02} & 0.19 \tn{.03}}{0.60 \tn{.02} & 0.60 \tn{.03} & 0.01 \tu{} & 0.04 \tp{.03}} \\
        & \row{DAE}{0.47 \tp{.03} & 0.68 \tp{.03} & 0.07 \tp{.02} & 0.15 \tp{.02}}{0.71 \tp{.01} & 0.75 \tp{.01} & 0.14 \tp{.01} & 0.20 \tu{}}{0.81 \tu{} & 0.81 \tp{.01} & 0.48 \tp{.01} & 0.50 \tp{.01}}{0.59 \tp{.05} & 0.60 \tp{.05} & 0.01 \tu{} & 0.03 \tu{}} \\
        & \row{CutPaste} {0.49 \tp{.11} & 0.71 \tp{.13} & 0.02 \tn{.01} & 0.04 \tn{.02}}{0.68 \tp{.07} & 0.73 \tp{.08} & 0.07 \tu{} & 0.13 \tu{}}{0.66 \tp{.07} & 0.70 \tp{.07} & 0.31 \tp{.09} & 0.35 \tp{.09}}{\textbf{0.70} \tp{.06} & \textbf{0.65} \tp{.05} & \textbf{0.04} \tp{.02} & \textbf{0.11} \tp{.05}} \\
        \cmidrule(r{4pt}){1-2}\cmidrule{3-6}\cmidrule{8-11}\cmidrule{13-16}\cmidrule{18-21}
        & \row{Random}{0.30  & 0.50  & 0.02  & 0.03}{0.48  & 0.50  & 0.06  & 0.11}{0.48  & 0.50  & 0.06  & 0.11}{0.50  & 0.50  & 0.004  & 0.01 } \\
        \bottomrule
    \end{tabular}}
\end{table*}


% Version 2
% \renewcommand{\row}[5]{ #1 & #4 && #3 && #2 && #5}
%     \begin{table*}
%     \centering
%     \caption{Detection and localization results of the image-reconstruction (\textbf{IR}), feature-modeling (\textbf{FM}), attention-based (\textbf{AB}), and self-supervised anomaly detection (\textbf{S-S}) methods on the brain-MRI and RF datasets after self-supervised pre-training.}
%     \label{tab:pretrain}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{clccccccccccccccccccc}
%         \toprule
%         % Datasets
%         & \row{}{\multicolumn{4}{c}{\textbf{ATLAS}}}{\multicolumn{4}{c}{\textbf{BraTS-T1}}}{\multicolumn{4}{c}{\textbf{BraTS-T2}}}{ \multicolumn{4}{c}{\textbf{DDR}}}\\
%         \cmidrule(r{4pt}){1-2}\cmidrule{3-6}\cmidrule{8-11}\cmidrule{13-16}\cmidrule{18-21}
%         % Metrics
%         & & \multicolumn{2}{c}{image-level} & \multicolumn{2}{c}{pixel-level} && \multicolumn{2}{c}{image-level} & \multicolumn{2}{c}{pixel-level} && \multicolumn{2}{c}{image-level} & \multicolumn{2}{c}{pixel-level} && \multicolumn{2}{c}{image-level} & \multicolumn{2}{c}{pixel-level} \\[1mm]
%         & Method & \api & AUROC & \app & \dice && \api & AUROC & \app & \dice && \api & AUROC & \app & \dice && \api & AUROC & \app & \dice \\
%         \cmidrule(r{4pt}){1-2}\cmidrule{3-6}\cmidrule{8-11}\cmidrule{13-16}\cmidrule{18-21}
%         % Image space methods
%         \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{IR}}}}
%         & \row{VAE}{0.57 & 0.76 & \textbf{0.11} & 0.20}{0.64 & 0.70 & 0.13 & 0.19}{0.68 & 0.73 & 0.27 & 0.33}{0.48 & 0.48 & 0.02 & 0.05} \\
%         & \row{r-VAE}{\textbf{0.61} & \textbf{0.79} & 0.09 & 0.17}{0.70 & 0.76 & 0.13 & 0.19}{0.75 & 0.77 & 0.36 & 0.40}{0.49 & 0.48 & 0.02 & 0.09} \\
%         & \row{f-AnoGAN}{0.28 & 0.50 & 0.02 & 0.04}{0.48 & 0.53 & 0.06 & 0.11}{0.63 & 0.70 & 0.15 & 0.21}{0.41 & 0.42 & 0.01 & 0.01} \\
%         & \row{H-TAE-S}{N/A & N/A & N/A & N/A}{N/A & N/A & N/A & N/A}{N/A & N/A & N/A & N/A}{N/A & N/A & N/A & N/A} \\
%         \cmidrule(r{4pt}){1-2}\cmidrule{3-6}\cmidrule{8-11}\cmidrule{13-16}\cmidrule{18-21}
%         % Feature space methods
%         \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{FM}}}}
%         & \row{FAE}{0.53 & 0.75 & 0.10 & \textbf{0.21}}{\textbf{0.85} & \textbf{0.85} & \textbf{0.43} & \textbf{0.46}}{\textbf{0.89} & \textbf{0.88}  &\textbf{0.55} & \textbf{0.55}}{0.55 & 0.57 & 0.03 & 0.08} \\
%         & \row{PaDiM}{0.41 & 0.65 & 0.07 & 0.16}{0.74 & 0.78 & 0.26 & 0.32}{0.81 & 0.81 & 0.47 & 0.48}{0.54 & 0.54 & 0.02 & 0.05} \\
%         & \row{CFLOW-AD}{0.45 & 0.68 & 0.06 & 0.14}{0.76 & 0.78 & 0.24 & 0.30}{0.79 & 0.80 & 0.31 & 0.38}{0.53 & 0.54 & 0.02 & 0.07} \\
%         & \row{RD}{0.42 & 0.64 & 0.05 & 0.09}{0.74 & 0.78 & 0.28 & 0.35}{0.84 & 0.85 & 0.39 & 0.44}{0.53 & 0.54 & \textbf{0.04} & 0.09} \\
%         \cmidrule(r{4pt}){1-2}\cmidrule{3-6}\cmidrule{8-11}\cmidrule{13-16}\cmidrule{18-21}
%         % Attention-based methods
%         \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{AB}}}}
       
%     & \row{ExpVAE} {0.40 & 0.62 & 0.01 & 0.03}{0.58 & 0.61 & 0.05 & 0.12}{0.66 & 0.68 & 0.15 & 0.22}{0.52 & 0.53 & 0.004 & 0.01}  \\

%         & \row{AMCons}{0.31 & 0.52 & 0.01 & 0.03}{0.61 & 0.64 & 0.06 & 0.12}{0.73 & 0.74 & 0.27 & 0.34}{0.49 & 0.50 & 0.004 & 0.01} \\
%         \cmidrule(r{4pt}){1-2}\cmidrule{3-6}\cmidrule{8-11}\cmidrule{13-16}\cmidrule{18-21}
%         % Self-supervised methods
%         \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{S-S}}}}
%         & \row{PII}{0.32 & 0.52 & 0.02 & 0.05}{0.46 & 0.50 & 0.07 & 0.14}{0.60 & 0.66 & 0.11 & 0.19}{0.60 & 0.60 & 0.01 & 0.04} \\
%         & \row{DAE}{0.47 & 0.68 & 0.07 & 0.15}{0.71 & 0.75 & 0.14 & 0.20}{0.81 & 0.81 & 0.48 & 0.50}{0.59 & 0.60 & 0.01 & 0.03} \\
%         & \row{CutPaste} {0.49 & 0.71 & 0.02 & 0.04}{0.68 & 0.73 & 0.07 & 0.13}{0.66 & 0.70 & 0.31 & 0.35}{\textbf{0.70} & \textbf{0.65} & \textbf{0.04} & \textbf{0.11}} \\
%         \cmidrule(r{4pt}){1-2}\cmidrule{3-6}\cmidrule{8-11}\cmidrule{13-16}\cmidrule{18-21}
%         & \row{Random}{0.30 & 0.50 & 0.02 & 0.03}{0.48 & 0.50 & 0.06 & 0.11}{0.48 & 0.50 & 0.06 & 0.11}{0.50 & 0.50 & 0.004 & 0.01} \\
%         \bottomrule
%     \end{tabular}}
% \end{table*}



% From first submission
% \begin{table*}
% \centering
% \caption{Detection and localization results of the compared methods on the brain-MRI and RF datasets after self-supervised pre-training.}
% \label{tab:pretrain}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{lccccccccccccccccccc}
% \toprule
%  & \multicolumn{4}{c}{\textbf{ATLAS}} &  & \multicolumn{4}{c}{\textbf{BraTS-T1}} &  & \multicolumn{4}{c}{\textbf{BraTS-T2}} &  & \multicolumn{4}{c}{\textbf{DDR}}\\
% \cmidrule(r{4pt}){1-1}\cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}\cmidrule{17-20}
% Method & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize} & \begin{scriptsize}$\lceil$Dice$\rceil$ \end{scriptsize}&  & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize} & \begin{scriptsize}$\lceil$Dice$\rceil$ \end{scriptsize}&  & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize} & \begin{scriptsize}$\lceil$Dice$\rceil$ \end{scriptsize}&  & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize} & \begin{scriptsize}$\lceil$Dice$\rceil$ \end{scriptsize}\\
% \cmidrule(r{4pt}){1-1}\cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}\cmidrule{17-20}
% VAE      & 0.57 & 0.76  & \textbf{0.11} & 0.20            &  & 0.64 & 0.70  & 0.13 & 0.19                 &  & 0.68 & 0.73  & 0.27 & 0.33                 &  & 0.48 & 0.48  & 0.02  & 0.05                  \\
% r-VAE    & \textbf{0.61} & \textbf{0.79}  & 0.09 & 0.17              &  & 0.70 & 0.76  & 0.13 & 0.19                 &  & 0.75 & 0.77  & 0.36 & 0.40                 &  & 0.49 & 0.48  & 0.02  & 0.09                  \\
% f-AnoGAN & 0.28 & 0.50  & 0.02 & 0.04                &  & 0.48 & 0.53  & 0.06 & 0.11                 &  & 0.63 & 0.70  & 0.15 & 0.21                 &  & 0.41 & 0.42  & 0.01  & 0.01                  \\
% AMCons   & 0.31 & 0.52  & 0.01 & 0.03               &  & 0.61 & 0.64  & 0.06 & 0.12                 &  & 0.73 & 0.74  & 0.27 & 0.34                 &  & 0.49 & 0.50  & 0.004  & 0.01                  \\
% FAE      & 0.53 & 0.75  & 0.10 & \textbf{0.21}                  &  & \textbf{0.85} & \textbf{0.85}  & \textbf{0.43} & \textbf{0.46}                 &  & \textbf{0.89} & \textbf{0.88}  &\textbf{0.55} & \textbf{0.55}                 &  & 0.55 & 0.57  & 0.03  & 0.08                  \\
% % DFR      & 0.46 & 0.70  & 0.07 & 0.18                   &  & 0.73 & 0.77  & 0.32 & 0.37                 &  & 0.76 & 0.78  & 0.46 & 0.47                 &  & 0.53 & 0.50  & 0.03  & 0.08                  \\
% PaDiM    & 0.41 & 0.65  & 0.07 & 0.16                  &  & 0.74 & 0.78  & 0.26 & 0.32                 &  & 0.81 & 0.81  & 0.47 & 0.48                 &  & 0.54 & 0.54  & 0.02  & 0.05                  \\
% CFLOW-AD & 0.45 & 0.68  & 0.06 & 0.14                 &  & 0.76 & 0.78  & 0.24 & 0.30                 &  & 0.79 & 0.80  & 0.31 & 0.38                 &  & 0.53 & 0.54  & 0.02  & 0.07                  \\
% RD       & 0.42 & 0.64  & 0.05 & 0.09              &  & 0.74 & 0.78  & 0.28 & 0.35                 &  & 0.84 & 0.85  & 0.39 & 0.44                 &  & 0.53 & 0.54  & \textbf{0.04}  & 0.09                  \\
% PII      & 0.32 & 0.52  & 0.02 & 0.05                  &  & 0.46 & 0.50  & 0.07 & 0.14                 &  & 0.60 & 0.66  & 0.11 & 0.19                 &  & \textbf{0.60} & \textbf{0.60}  & 0.01  & 0.04                  \\
% DAE      & 0.47 & 0.68  & 0.07 & 0.15                 &  & 0.71 & 0.75  & 0.14 & 0.20                 &  & 0.81 & 0.81  & 0.48 & 0.50                 &  & 0.59 & \textbf{0.60}  & 0.01  & 0.03                  \\
% Random   & 0.30 & 0.50  & 0.02 & 0.03                &  & 0.48 & 0.50  & 0.06 & 0.11                 &  & 0.48 & 0.50  & 0.06 & 0.11                 &  & 0.50 & 0.50  & 0.004 & 0.01                  \\
% \bottomrule
% \end{tabular}}
% \end{table*}





==> tables/pretrain_std.tex <==

\begin{table*}[htb]
\centering
\caption{Detection and localization results with standard deviation of selected methods on the MRI datasets after self-supervised pre-training.}
\label{tab:pretrain_std}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccccccccccccc}
\toprule
 & \multicolumn{4}{c}{\textbf{ATLAS}} &  & \multicolumn{4}{c}{\textbf{BraTS-T1}} &  & \multicolumn{4}{c}{\textbf{BraTS-T2}} \\
\cmidrule(r{4pt}){1-1}\cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}
Method & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize} & \begin{scriptsize}$\lceil$Dice$\rceil$ \end{scriptsize}&  & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize} & \begin{scriptsize}$\lceil$Dice$\rceil$ \end{scriptsize}&  & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize}& \begin{scriptsize}$\lceil$Dice$\rceil$ \end{scriptsize}\\
\cmidrule(r{4pt}){1-1}\cmidrule{2-5}\cmidrule{7-10}\cmidrule{12-15}
VAE      & 0.57
  \begin{scriptsize}(0.02)\end{scriptsize} & 0.76
  \begin{scriptsize}(0.01)\end{scriptsize} & 0.11
  \begin{scriptsize}(0.01)\end{scriptsize}                 & 0.20
  \begin{scriptsize}(0.02)\end{scriptsize} &~                     & 0.64
  \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.70
  \begin{scriptsize}(0.01)\end{scriptsize}                    & 0.13
  \begin{scriptsize}(0.01)\end{scriptsize}                 & 0.19
  \begin{scriptsize}(0.01)\end{scriptsize}                 & ~                     & 0.68
  \begin{scriptsize}(0.02)\end{scriptsize}                   & 0.73
  \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.27
  \begin{scriptsize}(0.02)\end{scriptsize}                   & 0.33
  \begin{scriptsize}(0.01)\end{scriptsize}                    \\
r-VAE   &  0.61
  \begin{scriptsize}(0.00)\end{scriptsize}   & 0.79 \begin{scriptsize}(0.00)\end{scriptsize}     & 0.09 \begin{scriptsize}(0.00)\end{scriptsize}                     & 0.17 \begin{scriptsize}(0.00)\end{scriptsize}    & ~                     & 0.70 \begin{scriptsize}(0.01)\end{scriptsize}                      & 0.76 \begin{scriptsize}(0.00)\end{scriptsize}                       & 0.13 \begin{scriptsize}(0.00)\end{scriptsize}                     & 0.19 \begin{scriptsize}(0.00)\end{scriptsize}                     & ~                     & 0.75 \begin{scriptsize}(0.00)\end{scriptsize}                        & 0.77 \begin{scriptsize}(0.00)\end{scriptsize}                        & 0.36 \begin{scriptsize}(0.01)\end{scriptsize}                        & 0.40 \begin{scriptsize}(0.01)\end{scriptsize}                          \\
f-AnoGAN & 0.28
  \begin{scriptsize}(0.01)\end{scriptsize} & 0.5 \begin{scriptsize}(0.03)\end{scriptsize}    & 0.02 \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.04 \begin{scriptsize}(0.02)\end{scriptsize}  &  ~                     & 0.48 \begin{scriptsize}(0.02)\end{scriptsize}                     & 0.53 \begin{scriptsize}(0.02)\end{scriptsize}                     & 0.06 \begin{scriptsize}(0.00)\end{scriptsize}                     & 0.11 \begin{scriptsize}(0.00)\end{scriptsize}                     & ~                     & 0.63 \begin{scriptsize}(0.02)\end{scriptsize}                     & 0.70 \begin{scriptsize}(0.02)\end{scriptsize}                      & 0.15 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.21 \begin{scriptsize}(0.00)\end{scriptsize}                        \\
AMCons  & 0.31
  \begin{scriptsize}(0.03)\end{scriptsize} & 0.52 \begin{scriptsize}(0.03)\end{scriptsize}   & \multicolumn{1}{l}{0.01 \begin{scriptsize}(0.00)\end{scriptsize}} & 0.03 \begin{scriptsize}(0.00)\end{scriptsize}    & \multicolumn{1}{l}{~} & \multicolumn{1}{l}{0.61 \begin{scriptsize}(0.01)\end{scriptsize}} & \multicolumn{1}{l}{0.64 \begin{scriptsize}(0.02)\end{scriptsize}} & \multicolumn{1}{l}{0.06 \begin{scriptsize}(0.00)\end{scriptsize}} & \multicolumn{1}{l}{0.12 \begin{scriptsize}(0.00)\end{scriptsize}} & \multicolumn{1}{l}{~} & \multicolumn{1}{l}{0.73 \begin{scriptsize}(0.05)\end{scriptsize}} & \multicolumn{1}{l}{0.74 \begin{scriptsize}(0.03)\end{scriptsize}} & \multicolumn{1}{l}{0.27 \begin{scriptsize}(0.07)\end{scriptsize}} & \multicolumn{1}{l}{0.34 \begin{scriptsize}(0.06)\end{scriptsize}}  \\
FAE      & 0.53
  \begin{scriptsize}(0.00)\end{scriptsize}   & 0.75 \begin{scriptsize}(0.00)\end{scriptsize}     & 0.10 \begin{scriptsize}(0.00)\end{scriptsize}                      & 0.21 \begin{scriptsize}(0.00)\end{scriptsize}    & ~                     & 0.85 \begin{scriptsize}(0.00)\end{scriptsize}                       & 0.85 \begin{scriptsize}(0.00)\end{scriptsize}                       & 0.43 \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.46 \begin{scriptsize}(0.00)\end{scriptsize}                     & ~                     & 0.89 \begin{scriptsize}(0.00)\end{scriptsize}                       & 0.88 \begin{scriptsize}(0.00)\end{scriptsize}                       & 0.55 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.55 \begin{scriptsize}(0.00)\end{scriptsize}                        \\
% DFR       & 0.46
%   \begin{scriptsize}(0.02)\end{scriptsize} & 0.70 \begin{scriptsize}(0.03)\end{scriptsize}    & 0.07 \begin{scriptsize}(0.00)\end{scriptsize}                     & 0.18 \begin{scriptsize}(0.01)\end{scriptsize}  & ~                     & 0.73 \begin{scriptsize}(0.02)\end{scriptsize}                     & 0.77 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.32 \begin{scriptsize}(0.02)\end{scriptsize}                   & 0.37 \begin{scriptsize}(0.01)\end{scriptsize}                   & ~                     & 0.76 \begin{scriptsize}(0.04)\end{scriptsize}                     & 0.78 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.46 \begin{scriptsize}(0.03)\end{scriptsize}                     & 0.47 \begin{scriptsize}(0.01)\end{scriptsize}                      \\
PaDiM    & 0.41
  \begin{scriptsize}(0.07)\end{scriptsize} & 0.65 \begin{scriptsize}(0.08)\end{scriptsize}   & 0.07 \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.16 \begin{scriptsize}(0.02)\end{scriptsize}  &  ~                     & 0.74 \begin{scriptsize}(0.04)\end{scriptsize}                     & 0.78 \begin{scriptsize}(0.02)\end{scriptsize}                     & 0.26 \begin{scriptsize}(0.06)\end{scriptsize}                   & 0.32 \begin{scriptsize}(0.04)\end{scriptsize}                   & ~                     & 0.81 \begin{scriptsize}(0.02)\end{scriptsize}                     & 0.81 \begin{scriptsize}(0.02)\end{scriptsize}                     & 0.47 \begin{scriptsize}(0.03)\end{scriptsize}                     & 0.48 \begin{scriptsize}(0.02)\end{scriptsize}                      \\
CFLOW-AD & 0.45
  \begin{scriptsize}(0.02)\end{scriptsize} & 0.68 \begin{scriptsize}(0.02)\end{scriptsize}   & 0.06 \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.14 \begin{scriptsize}(0.02)\end{scriptsize}  & ~                     & 0.76 \begin{scriptsize}(0.03)\end{scriptsize}                     & 0.78 \begin{scriptsize}(0.03)\end{scriptsize}                     & 0.24 \begin{scriptsize}(0.03)\end{scriptsize}                   & 0.30 \begin{scriptsize}(0.03)\end{scriptsize}                    & ~                     & 0.79 \begin{scriptsize}(0.00)\end{scriptsize}                       & 0.80 \begin{scriptsize}(0.00)\end{scriptsize}                        & 0.31 \begin{scriptsize}(0.03)\end{scriptsize}                     & 0.38 \begin{scriptsize}(0.02)\end{scriptsize}                      \\
RD       & 0.42
  \begin{scriptsize}(0.13)\end{scriptsize} & 0.64 \begin{scriptsize}(0.12)\end{scriptsize}   & 0.05 \begin{scriptsize}(0.06)\end{scriptsize}                   & 0.09 \begin{scriptsize}(0.10)\end{scriptsize}   & ~                     & 0.74 \begin{scriptsize}(0.03)\end{scriptsize}                     & 0.78 \begin{scriptsize}(0.02)\end{scriptsize}                     & 0.28 \begin{scriptsize}(0.02)\end{scriptsize}                   & 0.35 \begin{scriptsize}(0.02)\end{scriptsize}                   & ~                     & 0.84 \begin{scriptsize}(0.02)\end{scriptsize}                     & 0.85 \begin{scriptsize}(0.02)\end{scriptsize}                     & 0.39 \begin{scriptsize}(0.05)\end{scriptsize}                     & 0.44 \begin{scriptsize}(0.04)\end{scriptsize}                      \\
PII       & 0.32
  \begin{scriptsize}(0.02)\end{scriptsize} & 0.52 \begin{scriptsize}(0.05)\end{scriptsize}   & 0.02 \begin{scriptsize}(0.01)\end{scriptsize}                   & 0.05 \begin{scriptsize}(0.02)\end{scriptsize}  & ~                     & 0.46 \begin{scriptsize}(0.07)\end{scriptsize}                     & 0.50\begin{scriptsize}(0.10)\end{scriptsize}                       & 0.07 \begin{scriptsize}(0.03)\end{scriptsize}                   & 0.14 \begin{scriptsize}(0.03)\end{scriptsize}                   & ~                     & 0.60 \begin{scriptsize}(0.15)\end{scriptsize}                      & 0.66 \begin{scriptsize}(0.17)\end{scriptsize}                     & 0.11 \begin{scriptsize}(0.04)\end{scriptsize}                     & 0.19 \begin{scriptsize}(0.06)\end{scriptsize}                      \\
DAE      & 0.47
  \begin{scriptsize}(0.04)\end{scriptsize} & 0.68 \begin{scriptsize}(0.03)\end{scriptsize}   & 0.07 \begin{scriptsize}(0.02)\end{scriptsize}                   & 0.15 \begin{scriptsize}(0.02)\end{scriptsize}  & ~                     & 0.71 \begin{scriptsize}(0.03)\end{scriptsize}                     & 0.75 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.14 \begin{scriptsize}(0.02)\end{scriptsize}                   & 0.20 \begin{scriptsize}(0.01)\end{scriptsize}                    & ~                     & 0.81 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.81 \begin{scriptsize}(0.01)\end{scriptsize}                     & 0.48 \begin{scriptsize}(0.05)\end{scriptsize}                     & 0.50 \begin{scriptsize}(0.02)\end{scriptsize}                       \\
Random   & 0.26                                                                                                  & 0.50                                                                                                & 0.01                                                                                              & 0.02                                                                                              &                       & 0.48                                                                                                & 0.50                                                                                                & 0.06                                                                                              & 0.11                                                                                              &                       & 0.48                                                                                                & 0.50                                                                                                & 0.06                                                                                                & 0.11                                                                                                 \\
\bottomrule
\end{tabular}}
\end{table*}




==> tables/pretrain_std_2.tex <==
% \usepackage{caption}
% \usepackage{booktabs}



\begin{table*}[htb]
\centering
\caption{Detection and localization results with standard deviation of selected methods on the RF and CXR datasets after self-supervised pre-training.}
\label{tab:pretrain_std_2}
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccccccc} 
\toprule
 & \multicolumn{4}{c}{\textbf{DDR}}& \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{CheXpert - Pleural Effusion}}& & \multicolumn{2}{c}{\textbf{\textbf{CheXpert - Opacity}}}& \multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{CheXpert - Enlarged Card.}} \\ 
\cmidrule(r{4pt}){1-1}\cmidrule{2-5}\cmidrule{7-8}\cmidrule{10-11}\cmidrule{13-14}
Method & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & \begin{scriptsize}AP\textsubscript{p}\end{scriptsize} & \begin{scriptsize}$\lceil$Dice$\rceil$\end{scriptsize}&& \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} & & \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize} && \begin{scriptsize}AP\textsubscript{i}\end{scriptsize} & \begin{scriptsize}AUROC\end{scriptsize}\\ 
\cmidrule(lr){1-1}\cmidrule{2-5}\cmidrule{7-8}\cmidrule{10-11}\cmidrule{13-14}
VAE& 0.48
\begin{scriptsize}(0.01)\end{scriptsize} & 0.48
\begin{scriptsize}(0.02)\end{scriptsize} & 0.02
\begin{scriptsize}(0.00)\end{scriptsize} & 0.05
\begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.56
\begin{scriptsize}(0.00)\end{scriptsize} & 0.58
\begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.52
\begin{scriptsize}(0.00)\end{scriptsize} & 0.54
\begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.56
\begin{scriptsize}(0.00)\end{scriptsize} & 0.57
\begin{scriptsize}(0.00)\end{scriptsize}\\
r-VAE& 0.49
\begin{scriptsize}(0.04)\end{scriptsize} & 0.48 \begin{scriptsize}(0.03)\end{scriptsize} & 0.02 \begin{scriptsize}(0.02)\end{scriptsize} & 0.09 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.52
\begin{scriptsize}(0.00)\end{scriptsize} & 0.57 \begin{scriptsize}(0.01)\end{scriptsize} & ~& 0.47 \begin{scriptsize}(0.00)\end{scriptsize} & 0.49 \begin{scriptsize}(0.01)\end{scriptsize} & ~& 0.52 \begin{scriptsize}(0.02)\end{scriptsize} & 0.56 \begin{scriptsize}(0.02)\end{scriptsize}\\
f-AnoGAN & 0.41
\begin{scriptsize}(0.01)\end{scriptsize} & 0.42 \begin{scriptsize}(0.01)\end{scriptsize} & 0.01 \begin{scriptsize}(0.00)\end{scriptsize} & 0.01 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.60
\begin{scriptsize}(0.01)\end{scriptsize}& 0.62 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.50   \begin{scriptsize}(0.00)\end{scriptsize}& 0.52 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.58 \begin{scriptsize}(0.01)\end{scriptsize} & 0.60 \begin{scriptsize}(0.01)\end{scriptsize} \\
AMCons & 0.49
\begin{scriptsize}(0.02)\end{scriptsize} & 0.50 \begin{scriptsize}(0.00)\end{scriptsize}& 0.004 \begin{scriptsize}(0.00)\end{scriptsize} & 0.01 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.43
\begin{scriptsize}(0.05)\end{scriptsize} & 0.40 \begin{scriptsize}(0.08)\end{scriptsize}& ~& 0.50 \begin{scriptsize}(0.01)\end{scriptsize}& 0.52 \begin{scriptsize}(0.01)\end{scriptsize} & ~& 0.45 \begin{scriptsize}(0.04)\end{scriptsize} & 0.43 \begin{scriptsize}(0.06)\end{scriptsize}\\
FAE& 0.55
\begin{scriptsize}(0.02)\end{scriptsize} & 0.57 \begin{scriptsize}(0.01)\end{scriptsize} & 0.03 \begin{scriptsize}(0.00)\end{scriptsize} & 0.08 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.74
\begin{scriptsize}(0.00)\end{scriptsize} & 0.78 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.55 \begin{scriptsize}(0.00)\end{scriptsize} & 0.58 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.65 \begin{scriptsize}(0.00)\end{scriptsize} & 0.68 \begin{scriptsize}(0.00)\end{scriptsize}\\
% DFR& 0.53
% \begin{scriptsize}(0.00)\end{scriptsize} & 0.50 \begin{scriptsize}(0.00)\end{scriptsize}& 0.03 \begin{scriptsize}(0.00)\end{scriptsize} & 0.08 \begin{scriptsize}(0.01)\end{scriptsize} & ~& 0.51
% \begin{scriptsize}(0.01)\end{scriptsize} & 0.52 \begin{scriptsize}(0.01)\end{scriptsize} & ~~ & 0.45 \begin{scriptsize}(0.01)\end{scriptsize} & 0.45 \begin{scriptsize}(0.01)\end{scriptsize} & ~& 0.53 \begin{scriptsize}(0.01)\end{scriptsize} & 0.54 \begin{scriptsize}(0.01)\end{scriptsize}\\
PaDiM& 0.54
\begin{scriptsize}(0.02)\end{scriptsize} & 0.54 \begin{scriptsize}(0.01)\end{scriptsize} & 0.02 \begin{scriptsize}(0.00)\end{scriptsize} & 0.05 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.59
\begin{scriptsize}(0.01)\end{scriptsize} & 0.63 \begin{scriptsize}(0.01)\end{scriptsize} & ~& 0.48 \begin{scriptsize}(0.00)\end{scriptsize} & 0.49 \begin{scriptsize}(0.01)\end{scriptsize} & ~& 0.58 \begin{scriptsize}(0.00)\end{scriptsize} & 0.60 \begin{scriptsize}(0.01)\end{scriptsize} \\
CFLOW-AD & 0.53
\begin{scriptsize}(0.01)\end{scriptsize} & 0.54 \begin{scriptsize}(0.01)\end{scriptsize} & 0.02 \begin{scriptsize}(0.00)\end{scriptsize} & 0.07 \begin{scriptsize}(0.01)\end{scriptsize} & ~& 0.58
\begin{scriptsize}(0.01)\end{scriptsize} & 0.62 \begin{scriptsize}(0.01)\end{scriptsize} & ~& 0.47 \begin{scriptsize}(0.01)\end{scriptsize} & 0.48 \begin{scriptsize}(0.03)\end{scriptsize} & ~& 0.58 \begin{scriptsize}(0.00)\end{scriptsize} & 0.60 \begin{scriptsize}(0.01)\end{scriptsize} \\
RD & 0.53
\begin{scriptsize}(0.03)\end{scriptsize} & 0.54 \begin{scriptsize}(0.02)\end{scriptsize} & 0.04 \begin{scriptsize}(0.00)\end{scriptsize} & 0.09 \begin{scriptsize}(0.01)\end{scriptsize} & ~& 0.66
\begin{scriptsize}(0.02)\end{scriptsize} & 0.69 \begin{scriptsize}(0.02)\end{scriptsize} & ~& 0.55 \begin{scriptsize}(0.01)\end{scriptsize} & 0.58 \begin{scriptsize}(0.01)\end{scriptsize} & ~& 0.61 \begin{scriptsize}(0.01)\end{scriptsize} & 0.62 \begin{scriptsize}(0.01)\end{scriptsize}\\
PII& 0.60
\begin{scriptsize}(0.04)\end{scriptsize}& 0.60 \begin{scriptsize}(0.05)\end{scriptsize}& 0.01 \begin{scriptsize}(0.00)\end{scriptsize} & 0.04 \begin{scriptsize}(0.01)\end{scriptsize} & ~& 0.65
\begin{scriptsize}(0.03)\end{scriptsize} & 0.66 \begin{scriptsize}(0.03)\end{scriptsize} & ~& 0.52 \begin{scriptsize}(0.03)\end{scriptsize} & 0.53 \begin{scriptsize}(0.03)\end{scriptsize} & ~& 0.58 \begin{scriptsize}(0.02)\end{scriptsize} & 0.59 \begin{scriptsize}(0.02)\end{scriptsize}\\
DAE& 0.59
\begin{scriptsize}(0.05)\end{scriptsize} & 0.60 \begin{scriptsize}(0.04)\end{scriptsize}& 0.01 \begin{scriptsize}(0.00)\end{scriptsize} & 0.03 \begin{scriptsize}(0.01)\end{scriptsize} & ~& 0.62
\begin{scriptsize}(0.01)\end{scriptsize} & 0.64 \begin{scriptsize}(0.00)\end{scriptsize} & ~& 0.52 \begin{scriptsize}(0.01)\end{scriptsize} & 0.54 \begin{scriptsize}(0.01)\end{scriptsize} & ~& 0.58 \begin{scriptsize}(0.01)\end{scriptsize} & 0.60 \begin{scriptsize}(0.01)\end{scriptsize} \\
Random & 0.26& 0.50 & 0.004 & 0.01&& 0.50 & 0.50 && 0.50 & 0.50 && 0.50 & 0.50  \\
\bottomrule

\end{tabular}}
\end{table*}

==> tables/unused/encoder-level.tex <==
% \begin{table}[!b]

% \caption{Performance using different backbone layers}
% \label{tab:levels}
% \centering

% \begin{tabular}{ccccc}
%               & \multicolumn{2}{c}{MRI T2 (s)} & \multicolumn{2}{c}{MRI T2
%   (d)}  \\
%   \hline
%               & AP\textsubscript{i}    & AP\textsubscript{p}                       & AP\textsubscript{i}          & AP\textsubscript{p}                 \\ 
% \hline\\[-1.8ex] 
% \textbf{PaDiM} & 0.45    & \textbf{0.33}              & \textbf{0.59} & 0.15                 \\
% \textbf{CFLOW-AD} & 0.47    & \textbf{0.30}              & \textbf{0.50} & 0.25                 \\
% \textbf{RD} & 0.47    & \textbf{0.30}              & \textbf{0.50} & 0.25                \\ [0.2ex] 
% \hline 
%               &         &                            &               &                      \\
%               & \multicolumn{2}{c}{MRI T1 (s)} & \multicolumn{2}{c}{MRI T1 (d)}    \\
%               \hline
%               & AP\textsubscript{i}    & AP\textsubscript{p}                       & AP\textsubscript{i}          & AP\textsubscript{p}                  \\ 
% \hline\\[-1.8ex] 
% \textbf{PaDiM} & 0.24    & \textbf{0.08}              & \textbf{0.29} & 0.03                 \\
% \textbf{CFLOW-AD} & 0.22    & \textbf{0.07}              & 0.22          & 0.06                 \\ 
% \textbf{RD} & 0.47    & \textbf{0.30}              & \textbf{0.50} & 0.25                \\[0.2ex] 
% \hline 
%               &         &                            &               &                      \\
%               & CXR (s) & CXR (d)                    & RF (s)        & RF (d)               \\
%               \hline
%               & AP\textsubscript{i}    & AP\textsubscript{p}                       & AP\textsubscript{i}          & AP\textsubscript{p}                  \\ 
% \hline \\[-1.8ex] 
% \textbf{PaDiM} & 0.64    & \textbf{0.65}              & 0.59          & \textbf{0.62}        \\
% \textbf{CFLOW-AD} & 0.58    & \textbf{0.67}              & 0.62          & \textbf{0.67}        \\ 
% \textbf{RD} & 0.47    & \textbf{0.30}              & \textbf{0.50} & 0.25                
% \\ [0.2ex] \hline
% \end{tabular}
% \end{table}


% \usepackage{booktabs}


\begin{table*}[!t]
\centering
\caption{Performance using different backbone layers}
\label{tab:levels}
\resizebox{\linewidth}{!}{
\begin{tabular}{rccccccccccccccccc} 
\toprule
         & \multicolumn{2}{c}{MRI T2 (s)} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{MRI T2  (d)} &  & \multicolumn{2}{c}{MRI T1 (s)}                  &  & \multicolumn{2}{c}{MRI T1 (d)}                  &  & CXR (s) & CXR (d) &  & RF (s) & RF (d)  \\ 
\cmidrule{2-18}
         & APi  & APp                     &                      & APi           & APp             &  & APi                    & APp                    &  & APi                    & APp                    &  & APi     & APi     &  & APi    & APi     \\ 
\cmidrule{2-18}
PaDiM    & 0.45 & \textbf{0.33}           &                      & \textbf{0.59} & 0.15            &  & \textbf{\textbf{0.59}} & \textbf{\textbf{0.59}} &  & \textbf{\textbf{0.59}} & \textbf{\textbf{0.59}} &  & 0.25    & 0.25    &  & 0.25   & 0.25    \\
CFLOW-AD & 0.47 & \textbf{0.30}           &                      & \textbf{0.50} & 0.25            &  & \textbf{\textbf{0.59}} & \textbf{\textbf{0.59}} &  & \textbf{\textbf{0.59}} & \textbf{\textbf{0.59}} &  & 0.25    & 0.25    &  & 0.25   & 0.25    \\
RD       & 0.47 & \textbf{0.30}           &                      & \textbf{0.50} & 0.25            &  & \textbf{\textbf{0.59}} & \textbf{\textbf{0.59}} &  & \textbf{\textbf{0.59}} & \textbf{\textbf{0.59}} &  & 0.25    & 0.25    &  & 0.25   & 0.25     \\
\cmidrule[\heavyrulewidth]{1-18}
\end{tabular}}
\end{table*}

==> tables/unused/postproc.tex <==
% \begin{table*}[!t]
% \centering
% \caption{Performance using different backbone layers}
% \label{tab:IIIi}

% \begin{tabular}{ccccccccccccccc}
%                               & \multicolumn{4}{c}{IAP}                                                & \multicolumn{4}{c}{pap}                                                                   &                      &                           & \multicolumn{2}{c}{IAP}                     & \multicolumn{2}{c}{pAP}                      \\ 
% \cline{1-9}\cline{11-15}
% \textbf{}                     & abs/sq & \begin{tiny} SSIM \end{tiny}          & a/s+GB               & ssim + gb            & abs/sq               & \begin{tiny} SSIM \end{tiny}               & a/s+GB               & ssim + gb            &                      &                           & \begin{tiny}NO BLUR\end{tiny}               & \begin{tiny}BLUR\end{tiny}                & \begin{tiny}NO BLUR\end{tiny}               & \begin{tiny}BLUR\end{tiny}                 \\ 
% \cline{1-9}\cline{11-15} \\  [-1.8ex]
%  \textbf{VAE}       & 0.52   & 0.58            & 0.58                 & 0.62                 & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                      &  \textbf{PaDiM} & 0.52                 & 0.58                 & 0.52                 & 0.58                  \\
% \textbf{r-VAE}                & 0.52   & 0.58            & 0.58                 & 0.62                 & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                      & \textbf{CFLOW-AD}         & 0.52                 & 0.58                 & 0.52                 & 0.58                  \\
% \textbf{f-AnoGAN}             & 0.52   & 0.58            & 0.58                 & 0.62                 & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                      & \textbf{RD}               & 0.52                 & 0.58                 & 0.52                 & 0.58                  \\ 
% \cline{11-15}
% \textbf{DFR}           & 0.52        & 0.52 & 0.58                 & 0.62                 & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                      &                           &                      &                      &                      &                       \\ 
% \cline{1-9}
% \multicolumn{1}{c}{ } & \multicolumn{2}{c}{}     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}  \\
% \multicolumn{15}{c}{a) MRI T1}                                                                                                                                                                                                                                                                                                                     \\
% \multicolumn{15}{c}{}                                                                                                                                                                                                                                                                                                                              \\
% \textbf{}                     & \multicolumn{4}{c}{IAP}                                                & \multicolumn{4}{c}{pap}                                                                   &                      &                           & \multicolumn{2}{c}{IAP}                     & \multicolumn{2}{c}{pAP}                      \\ 
% \cline{1-9}\cline{11-15}
% \textbf{}                     & abs/sq & \begin{tiny} SSIM \end{tiny}          & a/s+GB               & ssim + gb            & abs/sq               & \begin{tiny} SSIM \end{tiny}               & a/s+GB               & ssim + gb            &                      &                           & \begin{tiny}NO BLUR\end{tiny}               & \begin{tiny}BLUR\end{tiny}                & \begin{tiny}NO BLUR\end{tiny}               & \begin{tiny}BLUR\end{tiny}                 \\ 
% \cline{1-9}\cline{11-15}\\  [-1.8ex]
%  \textbf{VAE}       & 0.52   & 0.58            & 0.58                 & 0.62                 & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                      &  \textbf{PaDiM} & 0.52                 & 0.58                 & 0.52                 & 0.58                  \\
% \textbf{r-VAE}                & 0.52   & 0.58            & 0.58                 & 0.62                 & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                      & \textbf{CFLOW-AD}         & 0.52                 & 0.58                 & 0.52                 & 0.58                  \\
% \textbf{f-AnoGAN}             & 0.52   & 0.58            & 0.58                 & 0.62                 & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                      & \textbf{RD}               & 0.52                 & 0.58                 & 0.52                 & 0.58                  \\ 
% \cline{11-15}
% \textbf{DFR}                  & 0.52   & 0.58            & 0.58                 & 0.62                 & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                      &                           &                      &                      &                      &                      \\
% \cline{1-9}
%                       &        &                 &                      &                      &                      &                      &                      &                      &                      &                           &                      &                      &                      &                       \\
% \multicolumn{15}{c}{b) MRI T2}                                                                                                                                                                                                                                                                                                                    
% \end{tabular}
% % \end{table*}
\begin{table*}[!t]
% \usepackage{booktabs}

% \usepackage{booktabs}

% \usepackage{booktabs}

% \usepackage{booktabs}


\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\centering
\caption{Effect of SSIM and post-processing.}
\label{tab:postproc}
\resizebox{\linewidth}{!}{%
\begin{tabular}{rP{0.8cm}P{0.8cm}P{0.8cm}P{0.8cm}cP{0.8cm}P{0.8cm}P{0.8cm}P{0.8cm}cP{0.8cm}P{0.8cm}cP{0.8cm}P{0.8cm}l}
\multicolumn{1}{c}{}          &      & \multicolumn{3}{c}{}                                               &                      & \multicolumn{4}{c}{}                                                                      & \multicolumn{1}{c}{} & \multicolumn{2}{c}{}                        &                      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &                    \\ 

\multicolumn{1}{c}{}          & \multicolumn{9}{c}{\textbf{ MRI T1}}                                                                                                                                                         & \multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{\textbf{MRI T1}}}                                                                     &                    \\ 
\cline{2-10}\cline{12-16}\\[-2.1ex]
\multicolumn{1}{c}{}          & \multicolumn{4}{c}{APi}                                                   & \multicolumn{1}{c}{} & \multicolumn{4}{c}{APp}                                                                   &                      & \multicolumn{2}{c}{IAP}                     & \multicolumn{1}{c}{} & \multicolumn{2}{c}{pAP}                     &                    \\ 
\cline{2-5}\cline{7-10}\cline{12-13}\cline{15-16}\\[-2.1ex]
\multicolumn{1}{c}{\textbf{}} & \begin{tiny}A/S\end{tiny}& \begin{tiny}SSIM\end{tiny}               & \begin{tiny} SSIM-GB \end{tiny}               & \begin{small} \begin{tiny}SSIM-GB\end{tiny} \end{small}              &                      & \begin{tiny}A/S\end{tiny}                & \begin{tiny} SSIM \end{tiny}               & \begin{tiny}SSIM-GB\end{tiny}               & \begin{small} \begin{tiny}SSIM-GB\end{tiny} \end{small}              &                      & \begin{tiny}NO BLUR\end{tiny}               & \begin{tiny}BLUR\end{tiny}                &                      & \begin{tiny}NO BLUR\end{tiny}               & \begin{tiny}BLUR\end{tiny}                &                    \\ 
\cline{2-5}\cline{7-10}\cline{12-13}\cline{15-16}
\textbf{VAE}                  & 0.00 & 0.58                 & 0.58                 & 0.62                 &                      & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                      & 0.52                 & 0.58                 &                      & 0.52                 & 0.58                 & \textbf{PaDiM}     \\
\textbf{r-VAE}                & 0.00 & 0.58                 & 0.58                 & 0.62                 &                      & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                      & 0.52                 & 0.58                 &                      & 0.52                 & 0.58                 & \textbf{CFLOW-AD}  \\
\textbf{f-AnoGAN}             & 0.00 & 0.58                 & 0.58                 & 0.62                 &                      & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                      & 0.52                 & 0.58                 &                      & 0.52                 & 0.58                 & \textbf{RD}        \\ 
\cline{12-16}
\textbf{DFR}                  & 0.00 & 0.52                 & 0.58                 & 0.62                 &                      & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                      &                      &                      &                      &                      &                      &                    \\ 
\cmidrule[\heavyrulewidth]{2-10}
\multicolumn{1}{c}{}          &      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &                      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &                      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &                    \\ 

\multicolumn{1}{c}{}          & \multicolumn{9}{c}{\textbf{ MRI T2}}                                                                                                                                                         & \multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{\textbf{MRI T2}}}                                                                     &                    \\ 
\cline{2-10}\cline{12-16}\\[-2.1ex]
\multicolumn{1}{c}{}          & \multicolumn{4}{c}{APi}                                                   & \multicolumn{1}{c}{} & \multicolumn{4}{c}{APp}                                                                   &                      & \multicolumn{2}{c}{IAP}                     & \multicolumn{1}{c}{} & \multicolumn{2}{c}{pAP}                     &                    \\ 
\cline{2-5}\cline{7-10}\cline{12-13}\cline{15-16}\\[-1.9ex]
\multicolumn{1}{c}{\textbf{}} & \begin{tiny}A/S\end{tiny}& \begin{tiny} SSIM \end{tiny}               & \begin{tiny} SSIM-GB \end{tiny}               & \begin{tiny} SSIM-GB \end{tiny}              &                      & \begin{tiny}A/S\end{tiny}                & \begin{tiny} SSIM \end{tiny}               & \begin{tiny} SSIM-GB \end{tiny}               & \begin{tiny} SSIM-GB \end{tiny}              &                      & \begin{tiny}NO BLUR\end{tiny}               & \begin{tiny}BLUR\end{tiny}                &                      & \begin{tiny}NO BLUR\end{tiny}               & \begin{tiny}BLUR\end{tiny}                &                    \\ 
\cline{2-5}\cline{7-10}\cline{12-13}\cline{15-16}\\[-1.9ex]
\textbf{VAE}                  & 0.00 & 0.58                 & 0.58                 & 0.62                 &                      & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                      & 0.52                 & 0.58                 &                      & 0.52                 & 0.58                 & \textbf{PaDiM}     \\
\textbf{r-VAE}                & 0.00 & 0.58                 & 0.58                 & 0.62                 &                      & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                      & 0.52                 & 0.58                 &                      & 0.52                 & 0.58                 & \textbf{CFLOW-AD}  \\
\textbf{f-AnoGAN}             & 0.00 & 0.58                 & 0.58                 & 0.62                 &                      & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                      & 0.52                 & 0.58                 &                      & 0.52                 & 0.58                 & \textbf{RD}        \\ 
\cline{12-16}
\textbf{DFR}                  & 0.00 & 0.58                 & 0.58                 & 0.62                 &                      & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                      &                      &                      &                      &                      &                      &                    \\
\cmidrule[\heavyrulewidth]{2-10}
\end{tabular}
}

\end{table*}


% \usepackage{color}
% \usepackage{booktabs}


% \begin{table*}
% \centering
% \caption{Effect of SSIM and post-processing.}
% \label{tab:postproc}
% \begin{tabular}{rp{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}lp{0.5cm}p{0.5cm}p{0.5cm}p{0.5cm}l}
% \multicolumn{1}{c}{}          &      & \multicolumn{3}{c}{}                                               &                      & \multicolumn{4}{c}{}                                                                      & \multicolumn{1}{c}{}                           \\ 
% \cmidrule[\heavyrulewidth]{2-10}
% \multicolumn{1}{c}{}          & \multicolumn{9}{c}{\textbf{ MRI T1}}                                                                                                                                                         & \multicolumn{1}{c}{}                           \\ 
% \cline{2-10}
% \multicolumn{1}{c}{}          & \multicolumn{4}{c}{APi}                                                   & \multicolumn{1}{c}{} & \multicolumn{4}{c}{APp}                                                                   &                                                \\ 
% \cline{2-5}\cline{7-10}
% \multicolumn{1}{c}{\textbf{}} & \begin{tiny}A/S\end{tiny}& \begin{tiny} SSIM \end{tiny}               & \begin{tiny} SSIM-GB \end{tiny}               & \begin{tiny} SSIM-GB \end{tiny}              &                      & \begin{tiny}A/S\end{tiny}                & \begin{tiny} SSIM \end{tiny}               & \begin{tiny} SSIM-GB \end{tiny}               & \begin{tiny} SSIM-GB \end{tiny}              &                                                \\ 
% \cline{2-5}\cline{7-10}
% \textbf{VAE}                  & 0.00 & 0.58                 & 0.58                 & 0.62                 &                      & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                                                \\
% \textbf{r-VAE}                & 0.00 & 0.58                 & 0.58                 & 0.62                 &                      & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                                                \\
% \textbf{f-AnoGAN}             & 0.00 & 0.58                 & 0.58                 & 0.62                 &                      & 0.15                 & 0.27                 & 0.37                 & 0.42                 & \textbf{\textbf{\textcolor{white}{f-AnoGAN}}}  \\
% \textbf{DFR}                  & 0.00 & 0.52                 & 0.58                 & 0.62                 &                      & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                                                \\ 
% \cmidrule[\heavyrulewidth]{2-10}
% \multicolumn{1}{c}{}          &      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &                      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                           \\ 
% \cmidrule[\heavyrulewidth]{2-10}
% \multicolumn{1}{c}{}          & \multicolumn{9}{c}{\textbf{ MRI T2}}                                                                                                                                                         & \multicolumn{1}{c}{}                           \\ 
% \cline{2-10}
% \multicolumn{1}{c}{}          & \multicolumn{4}{c}{APi}                                                   & \multicolumn{1}{c}{} & \multicolumn{4}{c}{APp}                                                                   &                                                \\ 
% \cline{2-5}\cline{7-10}
% \multicolumn{1}{c}{\textbf{}} & \begin{tiny}A/S\end{tiny}& \begin{tiny} SSIM \end{tiny}               & \begin{tiny} SSIM-GB \end{tiny}               & \begin{tiny} SSIM-GB \end{tiny}              &                      & \begin{tiny}A/S\end{tiny}                & \begin{tiny} SSIM \end{tiny}               & \begin{tiny} SSIM-GB \end{tiny}               & \begin{tiny} SSIM-GB \end{tiny}              &                                                \\ 
% \cline{2-5}\cline{7-10}
% \textbf{VAE}                  & 0.00 & 0.58                 & 0.58                 & 0.62                 &                      & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                                                \\
% \textbf{r-VAE}                & 0.00 & 0.58                 & 0.58                 & 0.62                 &                      & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                                                \\
% \textbf{f-AnoGAN}             & 0.00 & 0.58                 & 0.58                 & 0.62                 &                      & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                                                \\
% \textbf{DFR}                  & 0.00 & 0.58                 & 0.58                 & 0.62                 &                      & 0.15                 & 0.27                 & 0.37                 & 0.42                 &                                                \\
% \cmidrule[\heavyrulewidth]{2-10}
% \end{tabular}
% \end{table*}
